MONOS.II. Orbit review and analysis for 35 single-lined spectroscopic binary systems and candidates

[ABRIDGED] AIMS: The MONOS project is collecting information and studying O-type spectroscopic binaries with delta > -20 deg. In this 2nd paper, we tackle the study of the 35 single-line spectroscopic binary (SB1) systems identified in the previous paper of the series (arXiv:1904.11385) by analyzing our data and reviewing the literature orbits of such systems. METHODS: We have measured the radial velocities for the ~700 spectra in our database using two different methods: Gaussian fitting for several diagnostic lines per object and cross-correlation using synthetic spectra. We also explored the TESS database and analyzed the light curves for 31 of the systems. RESULTS: We have confirmed 21 SB1 systems, discarded the binary nature of 6 stars (9 Sge, HD 192 281, HDE 229 232 AB, 68 Cyg, HD 108 and \alpha Cam), and left 6 stars as inconclusive due to lack of data. The remaining two stars are 15 Mon Aa which has been classified as SB2, and Cyg OB2-22 C, for which we find evidence that it is most likely a triple system where the O star is orbiting an eclipsing SB1. We have also recalculated 20 new orbital solutions, including the first spectroscopic orbital solution for V747 Cep. For Cyg OB2-22 C we have obtained new ephemerides but no new orbit.

==> rvs.tex <==
\onecolumn

\begin{table}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~164\,438]{Radial velocity measurements for HD~164\,438. Errors in parenthesis corresponds to the last digit.\\
    \label{rvt:HD164438}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{6678}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} & \multicolumn{2}{c}{\SiIII{4553}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
080513\_F & 54\,600&896 & -1&6(1) & -0&1(2) & 1&8(4) & 3&3(3) & 4&1(9) & -1&2(5) & 5&8(5) & 4&4(13) \\
090524\_F & 54\,976&906 & -41&4(1) & -40&3(3) & -38&9(4) & -38&3(4) & -35&7(11) & -45&3(6) & -35&2(6) & -36&6(16) \\
100909\_I & 55\,449&360 & -46&6(1) & -47&3(2) & -45&5(5) & -46&7(3) & -43&9(11) & -45&1(5) & -42&2(4) & -44&6(14) \\
110515\_F & 55\,697&938 & -0&2(1) & 1&3(3) & 4&1(4) & 4&7(3) & 6&4(10) & -4&9(7) & 8&4(6) & 9&3(14) \\
110516\_F & 55\,698&852 & 5&0(1) & 6&5(3) & 8&1(4) & 10&3(3) & 11&1(11) & 0&9(7) & 13&3(6) & 8&6(15) \\
110614\_M & 55\,727&517 & -18&2(1) & -16&5(2) & -14&6(4) & -14&0(4) & -15&1(13) & -14&1(6) & -12&4(7) & -16&2(18) \\
110910\_I & 55\,815&394 & -14&4(1) & -14&5(2) & -13&0(4) & -12&0(3) & -10&5(12) & -10&7(5) & -8&8(4) & -11&4(13) \\
120519\_F & 56\,067&926 & 6&0(1) & 7&5(2) & 9&7(4) & 10&1(3) & 12&6(10) & 8&8(5) & 11&9(4) & 14&9(14) \\
130925\_C & 56\,561&307 & 0&8(1) & 4&1(4) & 6&0(6) & 5&0(8) & 5&7(26) & 6&9(11) & 11&3(11) & 10&4(35) \\
140606\_C & 56\,815&616 & 3&4(1) & 5&6(4) & 8&2(6) & 7&4(11) & 18&7(49) & 12&0(13) & 10&3(14) & 7&8(60) \\
140707\_C & 56\,846&556 & 5&2(1) & 7&2(4) & 10&0(6) & 10&4(9) & -0&9(37) & 9&1(10) & 12&7(11) & 10&5(42) \\
160721\_C & 57\,591&413 & -54&6(1) & -49&9(5) & -44&8(9) & -43&1(9) & -60&0(51) & -49&0(14) & -47&5(20) & -47&8(64) \\
170411\_S & 57\,855&714 & -21&0(1) & -19&5(3) & -17&7(6) & -17&7(7) & -20&2(23) & -16&6(9) & -17&2(8) & -17&8(22) \\
170606\_S & 57\,911&465 & -5&4(1) & -3&4(4) & -2&5(8) & 3&5(13) & .&. & 1&2(16) & 2&6(15) & 2&2(38) \\
170619\_S & 57\,924&484 & 1&8(1) & 3&8(3) & 5&3(7) & 9&8(9) & 4&2(29) & 7&4(11) & 8&6(9) & 7&1(30) \\
170706\_S & 57\,941&409 & -19&0(1) & -17&7(3) & -15&7(6) & -13&5(7) & -20&4(32) & -14&5(9) & -12&2(9) & -11&4(29) \\
170708\_S & 57\,943&408 & 7&2(1) & 9&4(3) & 12&3(6) & 13&7(8) & 7&7(24) & 10&9(9) & 14&5(10) & 18&9(20) \\
170709\_S & 57\,944&408 & 4&8(1) & 6&2(3) & 8&5(5) & 8&5(7) & 7&7(22) & 11&0(10) & 12&1(9) & 6&8(23) \\
170710\_S & 57\,945&407 & 1&2(1) & 2&0(3) & 5&2(6) & 4&7(7) & 1&8(20) & 5&1(8) & 6&7(8) & 7&3(24) \\
180727\_S & 58\,327&447 & -24&4(1) & -24&7(5) & -25&0(7) & -27&9(12) & -16&4(40) & -23&8(13) & -20&6(15) & -32&8(54) \\
190719\_C\_V & 58\,684&435 & -8&8(1) & -6&2(3) & -4&2(5) & -3&7(5) & .&. & -2&9(13) & -2&6(10) & .&. \\
190719\_C\_V\_2 & 58\,684&441 & -9&6(1) & -5&8(9) & -4&4(14) & -1&7(16) & .&. & -12&3(51) & -6&9(39) & .&. \\
190719\_C\_V\_3 & 58\,684&487 & -8&4(1) & -5&6(3) & -3&8(4) & -3&0(5) & .&. & -2&8(11) & -4&4(9) & .&. \\
190719\_C\_V\_4 & 58\,684&501 & -8&6(1) & -5&6(3) & -4&2(4) & -3&1(5) & .&. & -4&4(12) & -4&1(10) & .&. \\
\hline  RV mean & .&. & -10&3 & -8&5 & -6&5 & -2&0 & -4&6 & -7&3 & -4&0 & 3&2 \\
$\sigma$ RV & .&. & 16&8 & 17&0 & 16&9 & 13&2 & 16&9 & 17&6 & 17&5 & 10&8 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{4} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4144}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for V479~Sct]{Radial velocity measurements for V479~Sct. Errors in parenthesis corresponds to the last digit.\\
    \label{rvt:V479Sct}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{4686}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
000908\_P & 51\,796&315 & 17&0(1) & 23&0(27) & .&. & .&. & .&. & 27&7(32) & 43&8(70) \\
000912\_P & 51\,800&381 & 7&6(1) & 17&7(39) & .&. & .&. & .&. & 22&6(53) & .&. \\
010825\_P & 52\,147&361 & -21&8(1) & 22&3(29) & .&. & .&. & .&. & .&. & .&. \\
010826\_P & 52\,148&360 & 3&4(1) & 9&5(37) & .&. & .&. & .&. & .&. & .&. \\
010828\_P & 52\,150&351 & 4&8(1) & 3&2(27) & .&. & .&. & .&. & 13&1(36) & .&. \\
010829\_P & 52\,151&377 & -6&0(1) & 25&1(77) & .&. & .&. & .&. & .&. & .&. \\
010830\_P & 52\,152&325 & 34&4(1) & .&. & .&. & .&. & .&. & .&. & .&. \\
110415\_F & 55\,667&787 & 14&6(1) & 18&5(9) & 22&1(11) & 19&7(22) & 8&5(17) & 10&5(10) & 26&2(28) \\
110416\_F & 55\,668&794 & -9&4(1) & -2&2(8) & -2&4(10) & -4&6(20) & -12&8(14) & -10&6(8) & 12&5(30) \\
110417\_F & 55\,669&796 & 5&2(1) & 11&2(8) & 14&2(11) & 9&2(18) & 8&7(12) & 5&3(8) & 28&1(30) \\
110418\_F & 55\,670&857 & 23&8(1) & 27&0(9) & 32&9(10) & 27&0(18) & 27&0(13) & 22&2(8) & 46&3(32) \\
190318\_F & 58\,561&886 & 10&6(1) & 20&0(8) & 24&4(12) & 17&1(20) & 17&0(12) & 19&1(8) & 27&5(25) \\
190320\_F & 58\,563&859 & -11&0(1) & -5&0(8) & 2&4(12) & -6&5(16) & -11&9(10) & -4&9(8) & 8&4(25) \\
190320\_F\_2 & 58\,563&881 & -10&0(1) & -7&1(9) & 2&8(11) & -0&3(17) & -11&4(12) & -3&2(8) & 7&2(28) \\
190321\_F & 58\,564&851 & 24&6(1) & 31&1(8) & 38&1(11) & 32&0(15) & 23&9(11) & 29&0(7) & 43&6(22) \\
190901\_I & 58\,728&420 & 4&0(1) & 22&0(10) & 33&5(18) & .&. & -6&7(20) & 24&5(17) & 28&9(39) \\
191012\_I & 58\,769&336 & 3&0(1) & 9&3(12) & 21&2(16) & 13&8(32) & 2&6(19) & 16&2(13) & 29&1(37) \\
191014\_I & 58\,771&373 & 13&2(1) & 20&7(13) & 32&0(21) & 14&2(41) & 13&2(29) & 23&4(17) & 33&7(44) \\
\hline  RV mean & .&. & 6&0 & 14&5 & 20&1 & 12&2 & 5&3 & 13&9 & 27&9 \\
$\sigma$ RV & .&. & 13&9 & 11&2 & 13&4 & 12&2 & 13&8 & 12&3 & 12&7 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4471}, 5016, 5876, \HeII{4542}, 4686, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for 9~Sge]{Radial velocity measurements for 9~Sge. Errors in parenthesis corresponds to the last digit.\\
    \label{rvt:9Sge}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5801}} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5015}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
040530\_F & 53\,157&396 & 16&0(1) & 22&6(10) & 19&8(4) & 8&1(4) & -13&0(11) & 17&6(3) & 18&4(4) & 23&5(6) \\
040601\_F & 53\,159&357 & 24&4(1) & 30&0(8) & 27&6(4) & 17&3(4) & -9&9(14) & 25&8(4) & 28&1(4) & 31&0(6) \\
040827\_P & 53\,245&313 & 18&4(1) & 25&7(14) & 20&2(9) & 14&3(15) & -26&8(24) & 22&1(9) & 21&8(6) & 27&3(6) \\
051110\_P & 53\,685&253 & 21&2(1) & 26&5(14) & 21&6(11) & 13&0(14) & -2&1(21) & 20&4(10) & 21&1(8) & 25&8(16) \\
060624\_F & 53\,912&408 & 10&0(1) & 22&9(9) & 17&8(8) & 2&9(6) & -30&0(16) & 18&9(5) & 13&3(4) & 20&5(4) \\
060625\_F & 53\,913&397 & 12&8(1) & 22&1(10) & 15&7(7) & 5&5(5) & -22&1(12) & 18&5(4) & 15&0(4) & 21&1(4) \\
060626\_F & 53\,914&395 & 16&6(1) & 23&1(10) & 16&8(7) & 8&8(4) & -14&4(13) & 21&0(4) & 18&8(4) & 23&2(4) \\
091111\_I & 55\,147&880 & 8&4(1) & 21&7(9) & 17&0(5) & 10&1(4) & -24&1(11) & 16&1(4) & 20&0(3) & 22&3(3) \\
101024\_I & 55\,494&884 & 23&6(1) & 28&4(9) & 25&8(4) & 16&1(4) & -3&4(9) & 26&7(5) & 28&2(3) & 28&0(3) \\
110614\_M & 55\,727&982 & 20&0(1) & 27&3(9) & 23&1(5) & 12&7(4) & -24&7(10) & 24&5(4) & 25&0(3) & 26&5(10) \\
110614\_M\_2 & 55\,728&065 & 20&6(1) & 26&1(7) & 23&7(4) & 15&8(4) & -20&7(10) & 23&4(4) & 23&5(3) & 26&5(3) \\
110614\_M\_3 & 55\,728&149 & 21&8(1) & 29&2(7) & 25&3(4) & 17&3(4) & -14&1(10) & 23&0(4) & 24&5(3) & 29&6(3) \\
110614\_M\_4 & 55\,728&240 & 20&8(1) & 30&5(8) & 25&6(4) & 14&3(4) & -12&1(9) & 24&0(4) & 24&7(3) & 30&3(4) \\
110615\_M & 55\,728&974 & 16&4(1) & 25&3(7) & 23&3(4) & 8&8(4) & -17&7(8) & 21&5(4) & 21&0(3) & 23&0(6) \\
110615\_M\_2 & 55\,729&066 & 16&8(1) & 24&9(6) & 22&1(4) & 11&3(4) & -15&7(8) & 21&6(4) & 20&9(3) & 23&3(3) \\
110615\_M\_3 & 55\,729&151 & 17&6(1) & 27&4(7) & 23&8(3) & 11&2(4) & -13&1(8) & 23&4(4) & 21&8(2) & 24&6(3) \\
110616\_M & 55\,729&975 & 12&6(1) & 23&3(7) & 20&5(5) & 4&8(4) & -23&3(10) & 19&2(5) & 19&0(3) & 18&7(7) \\
110616\_M\_2 & 55\,730&069 & 12&0(1) & 20&6(7) & 17&8(4) & 4&9(3) & -25&2(9) & 17&4(4) & 16&4(2) & 18&6(3) \\
110616\_M\_3 & 55\,730&155 & 13&6(1) & 21&1(6) & 18&2(3) & 8&9(4) & -25&5(10) & 17&6(3) & 16&8(3) & 20&5(3) \\
110616\_M\_4 & 55\,730&246 & 16&6(1) & 24&9(7) & 21&9(4) & 10&5(4) & -23&5(10) & 20&9(4) & 20&7(3) & 24&5(3) \\
110617\_M & 55\,730&972 & 18&6(1) & 25&7(8) & 22&8(5) & 13&5(4) & -16&2(10) & 22&2(4) & 21&8(3) & 27&1(4) \\
110617\_M\_2 & 55\,731&005 & 20&4(1) & 27&7(8) & 24&3(4) & 15&6(4) & -15&9(10) & 23&5(4) & 23&4(3) & 28&0(4) \\
110617\_M\_3 & 55\,731&062 & 21&4(1) & 29&0(8) & 24&8(5) & 16&9(4) & -16&2(10) & 24&9(4) & 24&8(3) & 29&6(3) \\
110617\_M\_4 & 55\,731&118 & 20&2(1) & 27&9(8) & 24&9(4) & 15&5(4) & -16&1(10) & 23&6(4) & 24&2(3) & 27&2(4) \\
110617\_M\_5 & 55\,731&166 & 18&8(1) & 27&3(8) & 22&5(5) & 13&1(4) & -15&0(10) & 21&7(4) & 22&7(3) & 25&5(4) \\
110617\_M\_6 & 55\,731&233 & 15&0(1) & 23&2(8) & 17&8(5) & 9&2(4) & -15&9(10) & 17&4(4) & 17&6(3) & 21&7(4) \\
110618\_M & 55\,731&983 & 18&2(1) & 23&5(7) & 19&9(6) & 13&9(6) & -9&2(9) & 20&4(5) & 20&9(3) & 24&1(4) \\
110618\_M\_2 & 55\,732&022 & 16&6(1) & 23&4(7) & 20&6(9) & 12&1(6) & -11&4(10) & 20&6(6) & 19&4(4) & 22&1(5) \\
110618\_M\_3 & 55\,732&080 & 12&8(1) & 19&7(7) & 16&0(4) & 8&3(4) & -15&7(9) & 16&2(4) & 15&5(3) & 20&1(3) \\
110618\_M\_4 & 55\,732&133 & 9&6(1) & 18&4(7) & 15&2(4) & 4&7(5) & -20&4(9) & 14&4(4) & 12&7(3) & 16&6(3) \\
110618\_M\_5 & 55\,732&189 & 8&2(1) & 17&4(7) & 14&9(4) & 3&4(4) & -24&2(9) & 14&4(4) & 11&6(3) & 16&0(5) \\
110619\_M & 55\,732&974 & 11&8(1) & 18&8(7) & 16&3(4) & 4&3(4) & -26&5(10) & 17&1(4) & 15&1(3) & 17&8(4) \\
110619\_M\_2 & 55\,733&012 & 14&8(1) & 21&4(7) & 19&2(4) & 8&1(4) & -25&7(10) & 19&1(4) & 19&3(3) & 20&8(3) \\
110619\_M\_3 & 55\,733&072 & 19&2(1) & 26&1(7) & 22&5(4) & 11&8(3) & -22&2(11) & 22&5(4) & 23&8(3) & 24&7(3) \\
110619\_M\_4 & 55\,733&111 & 20&8(1) & 27&8(6) & 24&4(4) & 12&9(3) & -18&8(11) & 23&1(4) & 25&1(3) & 26&2(3) \\
110619\_M\_5 & 55\,733&162 & 23&4(1) & 28&3(7) & 25&1(4) & 16&0(3) & -12&4(10) & 23&8(4) & 26&4(3) & 28&0(3) \\
110619\_M\_6 & 55\,733&217 & 25&4(1) & 29&7(6) & 27&0(3) & 18&8(3) & -6&1(10) & 26&1(3) & 28&1(3) & 29&5(4) \\
110620\_M & 55\,733&951 & 24&6(1) & 32&3(7) & 29&3(5) & 18&6(4) & -8&5(10) & 27&7(5) & 29&6(4) & 31&4(8) \\
110620\_M\_2 & 55\,733&975 & 23&4(1) & 30&7(7) & 27&3(4) & 17&4(4) & -9&0(10) & 27&0(4) & 28&9(3) & 30&2(4) \\
110620\_M\_3 & 55\,734&036 & 19&0(1) & 27&1(8) & 22&8(4) & 10&8(4) & -13&1(10) & 23&5(4) & 23&9(3) & 25&4(4) \\
110711\_M & 55\,755&072 & 23&4(1) & 29&9(8) & 24&6(5) & 14&3(4) & -12&3(9) & 24&1(4) & 26&7(3) & 29&9(4) \\
110711\_M\_2 & 55\,755&170 & 17&2(1) & 23&9(7) & 20&0(4) & 9&7(4) & -11&7(9) & 20&6(4) & 20&9(3) & 21&5(4) \\
110712\_M & 55\,756&042 & 25&0(1) & 30&4(7) & 26&9(4) & 18&4(4) & -16&6(10) & 26&9(4) & 30&2(3) & 30&3(4) \\
110712\_M\_2 & 55\,756&149 & 25&2(1) & 30&3(8) & 24&1(4) & 18&3(4) & -12&5(10) & 27&2(4) & 29&1(3) & 30&0(4) \\
110714\_M & 55\,757&966 & 29&2(1) & 33&6(7) & 29&1(4) & 24&6(4) & 3&9(9) & 28&4(4) & 32&3(3) & 35&9(4) \\
110714\_M\_2 & 55\,758&090 & 18&8(1) & 24&9(7) & 20&0(5) & 13&9(7) & -7&7(10) & 19&9(4) & 21&6(3) & 27&0(5) \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4388}, 4713, 4922, \HeII{4200}, 4542, 5412, \HeI{}+\HeII{4026} and H$\gamma$+\HeII{4338}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\captionsetup[table]{list=no}
\addtocounter{table}{-1}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Continued.}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5801}} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5015}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
110908\_I & 55\,813&937 & 22&0(1) & 26&4(10) & 24&4(6) & 14&1(7) & -24&7(13) & 28&6(7) & 28&6(5) & 28&6(5) \\
110908\_I\_2 & 55\,814&078 & 22&6(1) & 27&5(9) & 25&3(5) & 13&7(5) & -23&3(14) & 27&7(5) & 26&6(4) & 27&7(4) \\
110909\_I & 55\,814&841 & 13&4(1) & 17&4(9) & 18&6(4) & 7&4(6) & -36&7(13) & 19&1(6) & 16&6(4) & 21&0(4) \\
110909\_I\_2 & 55\,814&910 & 13&8(1) & 20&1(9) & 19&9(5) & 6&0(5) & -38&7(12) & 20&2(6) & 18&4(4) & 21&0(4) \\
110909\_I\_3 & 55\,814&978 & 14&0(1) & 17&7(10) & 18&9(4) & 5&5(6) & -39&4(12) & 21&7(7) & 19&0(4) & 21&5(4) \\
110909\_I\_4 & 55\,815&038 & 13&0(1) & 17&3(10) & 17&3(5) & 5&8(6) & -42&6(12) & 19&7(6) & 17&6(4) & 22&2(4) \\
110910\_I & 55\,815&837 & 16&8(1) & 22&9(10) & 24&0(5) & 9&6(8) & -49&8(19) & 23&1(6) & 22&5(4) & 26&5(4) \\
110910\_I\_2 & 55\,815&915 & 16&6(1) & 22&6(10) & 24&3(5) & 8&2(7) & -51&6(19) & 24&3(6) & 22&8(4) & 25&8(5) \\
110910\_I\_3 & 55\,815&984 & 15&6(1) & 21&0(11) & 25&9(4) & 7&4(9) & -52&1(20) & 23&7(6) & 23&0(5) & 24&1(4) \\
110911\_I & 55\,816&836 & 19&8(1) & 21&0(10) & 22&9(4) & 13&4(6) & -15&4(15) & 22&4(7) & 23&7(5) & 25&3(4) \\
110911\_I\_2 & 55\,816&910 & 20&2(1) & 22&7(10) & 24&2(5) & 13&1(5) & -13&7(15) & 24&0(6) & 23&7(4) & 25&2(4) \\
110911\_I\_3 & 55\,816&994 & 21&0(1) & 22&6(9) & 22&4(5) & 15&7(5) & -8&6(13) & 23&9(6) & 24&2(3) & 25&9(4) \\
110911\_I\_4 & 55\,817&043 & 21&2(1) & 23&9(10) & 20&9(5) & 13&6(5) & -7&2(12) & 23&4(6) & 23&7(3) & 26&8(4) \\
121025\_M & 56\,226&816 & 10&2(1) & 18&8(8) & 15&1(4) & 1&5(5) & -20&2(7) & 15&6(4) & 14&3(3) & 18&3(4) \\
121025\_M\_2 & 56\,226&864 & 9&0(1) & 19&5(8) & 14&3(4) & 1&0(5) & -19&6(7) & 14&8(4) & 12&7(3) & 15&7(4) \\
121025\_M\_3 & 56\,226&915 & 8&2(1) & 17&7(7) & 13&5(4) & -0&3(6) & -21&3(7) & 13&4(4) & 11&4(3) & 14&8(4) \\
121025\_M\_4 & 56\,226&955 & 9&2(1) & 18&7(8) & 15&1(5) & -0&0(5) & -20&5(7) & 15&1(4) & 13&2(4) & 15&3(4) \\
121026\_M & 56\,227&805 & 18&0(1) & 27&8(7) & 23&5(4) & 12&0(4) & -5&2(9) & 21&1(4) & 21&4(3) & 26&1(3) \\
121026\_M\_2 & 56\,227&858 & 15&6(1) & 25&1(7) & 22&1(4) & 10&0(4) & -10&7(9) & 20&2(4) & 18&9(3) & 23&7(4) \\
130819\_C & 56\,524&883 & 13&2(1) & .&. & 29&6(17) & 22&7(48) & 2&2(18) & 30&4(37) & 5&6(34) & 34&1(18) \\
130920\_M & 56\,557&026 & 12&2(1) & 18&5(7) & 15&5(9) & 7&1(5) & -18&3(7) & 16&5(5) & 15&8(3) & 19&0(4) \\
130920\_M\_2 & 56\,557&066 & 12&6(1) & 21&1(7) & 19&0(5) & 6&8(5) & -19&3(7) & 17&7(5) & 17&2(4) & 18&6(4) \\
130921\_M & 56\,557&863 & 13&8(1) & 20&7(8) & 18&2(5) & 9&1(5) & -12&7(6) & 16&5(5) & 15&0(4) & 19&7(5) \\
130921\_M\_2 & 56\,557&942 & 13&4(1) & 21&0(8) & 18&0(6) & 7&5(6) & -14&5(7) & 18&0(5) & 16&0(4) & 20&9(5) \\
130922\_M & 56\,558&839 & 16&2(1) & 24&2(7) & 21&9(5) & 9&2(4) & -6&6(9) & 21&1(6) & 18&6(3) & 22&7(4) \\
130922\_M\_2 & 56\,558&905 & 16&0(1) & 24&5(8) & 22&4(5) & 7&0(5) & -6&0(8) & 19&8(4) & 19&1(3) & 21&2(4) \\
130923\_M & 56\,559&840 & 20&0(1) & 29&0(7) & 24&4(5) & 15&2(5) & -14&0(10) & 22&8(4) & 22&8(4) & 28&3(5) \\
130923\_M\_2 & 56\,559&903 & 17&6(1) & 26&3(7) & 23&0(5) & 11&1(5) & -15&5(9) & 20&7(5) & 20&2(4) & 25&4(5) \\
130926\_M & 56\,562&844 & 18&8(1) & 24&6(8) & 21&8(6) & 11&0(5) & -2&9(7) & 19&1(6) & 21&6(6) & 23&4(5) \\
130926\_M\_2 & 56\,562&972 & 17&4(1) & 25&0(8) & 22&2(6) & 11&5(6) & -1&7(7) & 19&8(5) & 20&0(4) & 22&4(5) \\
130927\_M & 56\,563&829 & 8&6(1) & 20&1(8) & 15&3(5) & 2&5(5) & -22&3(8) & 13&8(5) & 11&5(3) & 17&0(4) \\
130927\_M\_2 & 56\,563&950 & 9&6(1) & 19&8(7) & 16&4(5) & 5&4(5) & -21&7(8) & 15&8(5) & 12&0(3) & 17&3(4) \\
130928\_M & 56\,564&840 & 15&0(1) & 23&9(8) & 19&8(5) & 9&8(5) & -15&2(8) & 20&3(4) & 19&2(3) & 22&9(4) \\
130928\_M\_2 & 56\,564&896 & 14&4(1) & 23&1(8) & 19&6(5) & 7&0(5) & -15&5(7) & 18&5(4) & 19&6(3) & 18&6(5) \\
130928\_M\_3 & 56\,564&970 & 13&0(1) & 22&2(8) & 20&8(7) & 5&7(7) & -15&9(9) & 17&7(6) & 16&9(4) & 19&8(6) \\
130929\_M & 56\,565&828 & 7&2(1) & 17&0(9) & 14&4(5) & -1&2(5) & -23&3(8) & 12&7(5) & 11&0(3) & 15&5(5) \\
130929\_M\_2 & 56\,565&878 & 8&6(1) & 19&6(8) & 16&9(6) & -0&6(5) & -24&7(8) & 16&0(5) & 12&1(4) & 16&1(5) \\
130929\_M\_3 & 56\,565&983 & 11&0(1) & 19&8(8) & 18&6(6) & 2&3(5) & -22&3(8) & 17&9(5) & 15&7(3) & 17&8(5) \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\addtocounter{table}{-1}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Continued.}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5801}} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5015}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
130930\_M & 56\,566&826 & 21&6(1) & 29&6(7) & 25&7(5) & 16&6(5) & -18&3(11) & 25&6(5) & 27&8(3) & 28&9(5) \\
131024\_M & 56\,590&814 & 12&8(1) & 21&8(8) & 19&0(6) & 6&9(6) & -12&3(8) & 17&2(6) & 18&8(4) & 21&4(6) \\
131024\_M\_2 & 56\,590&856 & 12&8(1) & 21&8(7) & 18&9(4) & 7&0(4) & -13&3(8) & 17&4(4) & 17&3(3) & 20&2(3) \\
131024\_M\_3 & 56\,590&905 & 15&6(1) & 14&2(40) & 17&6(59) & 2&4(69) & -14&2(29) & 24&9(61) & 12&7(37) & 21&4(56) \\
131026\_M & 56\,592&821 & 23&6(1) & 28&3(7) & 24&3(5) & 17&6(4) & 7&6(7) & 23&7(4) & 25&0(3) & 29&9(4) \\
131026\_M\_2 & 56\,592&884 & 22&8(1) & 27&2(7) & 23&0(4) & 15&7(4) & 4&7(6) & 22&7(4) & 24&4(3) & 28&5(3) \\
131026\_M\_3 & 56\,592&928 & 23&0(1) & 30&1(8) & 25&6(7) & 16&5(6) & 3&8(7) & 24&4(7) & 25&7(5) & 27&4(6) \\
131027\_M & 56\,593&832 & 15&0(1) & 23&7(8) & 21&0(5) & 7&5(5) & -13&5(8) & 19&5(4) & 18&6(3) & 23&4(4) \\
131027\_M\_2 & 56\,593&880 & 15&0(1) & 24&9(8) & 21&8(5) & 8&0(4) & -15&2(7) & 20&6(4) & 18&9(3) & 22&5(4) \\
131027\_M\_3 & 56\,593&923 & 11&8(1) & 32&8(35) & 24&4(51) & 7&4(48) & -17&4(24) & 10&1(58) & 19&9(28) & 24&2(43) \\
131028\_M & 56\,594&812 & 14&2(1) & 23&4(7) & 20&5(5) & 7&0(4) & -12&0(7) & 19&1(6) & 18&9(3) & 20&5(3) \\
131028\_M\_2 & 56\,594&859 & 17&2(1) & 24&4(7) & 21&5(4) & 10&0(4) & -8&3(7) & 20&9(4) & 21&2(3) & 21&4(3) \\
131028\_M\_3 & 56\,594&924 & 20&6(1) & 27&2(8) & 24&0(4) & 13&3(4) & -3&7(7) & 22&5(4) & 23&8(3) & 25&4(3) \\
131029\_M & 56\,595&903 & 10&2(1) & 18&7(8) & 15&8(6) & 4&2(6) & -17&3(8) & 16&1(6) & 13&4(4) & 16&8(6) \\
131030\_M & 56\,596&802 & 11&8(1) & 17&5(8) & 15&3(6) & 5&6(6) & -9&1(7) & 13&3(6) & 14&8(4) & 18&0(5) \\
131030\_M\_2 & 56\,596&882 & 4&8(1) & 11&0(11) & 9&7(10) & -2&5(7) & -20&2(7) & 10&4(7) & 7&1(5) & 10&8(7) \\
150329\_C & 57\,112&209 & 15&8(1) & 26&2(13) & 20&1(13) & 8&0(15) & -7&6(13) & 17&6(11) & 20&4(8) & 24&0(11) \\
150531\_M & 57\,175&097 & 23&8(1) & 33&9(8) & 31&2(5) & 16&9(5) & -16&2(11) & 29&2(5) & 28&6(3) & 32&5(4) \\
160718\_C & 57\,589&018 & 19&0(1) & 29&4(11) & 26&7(8) & 17&7(12) & 4&2(11) & 19&5(9) & 25&0(6) & 29&0(8) \\
181211\_S & 58\,464&861 & 16&2(1) & 23&8(13) & 17&7(11) & 7&6(15) & -6&7(12) & 18&2(9) & 17&4(6) & 21&4(10) \\
190722\_C\_V & 58\,688&014 & 30&8(1) & 27&0(11) & 23&9(5) & .&. & -1&0(8) & .&. & 24&5(6) & 23&9(8) \\
190722\_C\_V\_2 & 58\,688&020 & 31&6(1) & 27&4(11) & 22&8(6) & .&. & -1&3(8) & .&. & 25&0(55) & 24&3(8) \\
\hline  RV mean & .&. & 16&9 & 24&2 & 21&2 & 10&2 & -15&0 & 20&7 & 20&3 & 23&7 \\
$\sigma$ RV & .&. & 5&3 & 4&4 & 4&0 & 5&4 & 9&3 & 4&1 & 5&2 & 4&7 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\captionsetup[table]{list=yes}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for Cyg~X-1]{Radial velocity measurements for Cyg~X-1. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:CygX-1}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} & \multicolumn{2}{c}{\SiIII{4553}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
081106\_I & 54\,777&342 & 31&8(1) & 27&3(30) & 16&9(6) & 31&5(6) & 44&6(27) & 50&1(12) & 44&1(11) & 22&9(31) \\
081106\_I\_2 & 54\,777&353 & 33&6(1) & 30&5(28) & 18&1(6) & 33&4(6) & 43&8(23) & 47&5(11) & 51&2(12) & 24&2(29) \\
081108\_I & 54\,779&306 & 15&6(1) & -0&2(42) & 6&4(4) & 15&3(7) & 22&8(32) & 30&4(14) & 34&0(16) & .&. \\
081108\_I\_2 & 54\,779&317 & 14&8(1) & -8&5(46) & 6&2(5) & 15&2(8) & 26&2(54) & 33&2(17) & 29&3(25) & .&. \\
110521\_H\_B & 55\,703&820 & -21&6(1) & .&. & .&. & .&. & -19&7(29) & .&. & .&. & -17&0(20) \\
110521\_H\_G & 55\,703&820 & -17&2(1) & .&. & .&. & .&. & .&. & -15&8(13) & -11&8(18) & .&. \\
110521\_H\_R & 55\,703&827 & -22&8(1) & .&. & .&. & -23&5(10) & .&. & .&. & .&. & .&. \\
110521\_H\_V & 55\,703&827 & -18&6(1) & -30&4(44) & -28&0(6) & .&. & .&. & -18&0(18) & -12&0(27) & .&. \\
110622\_H\_R & 55\,735&764 & 68&0(1) & .&. & .&. & 68&9(12) & .&. & .&. & .&. & .&. \\
110622\_H\_V & 55\,735&764 & 71&6(1) & 76&6(51) & 62&5(8) & .&. & .&. & 84&0(17) & 90&1(26) & .&. \\
111006\_H\_B & 55\,841&687 & 63&4(1) & .&. & .&. & .&. & 75&1(38) & .&. & .&. & 70&8(27) \\
111006\_H\_G & 55\,841&687 & 70&0(1) & .&. & .&. & .&. & .&. & 79&7(16) & 70&3(25) & .&. \\
111006\_H\_R & 55\,841&700 & 68&0(1) & .&. & .&. & 69&4(18) & .&. & .&. & .&. & .&. \\
111006\_H\_V & 55\,841&700 & 67&2(1) & .&. & 57&4(11) & .&. & .&. & 72&3(36) & 75&3(61) & .&. \\
111011\_H\_B & 55\,846&690 & 22&6(1) & .&. & .&. & .&. & 30&0(27) & .&. & .&. & 18&3(20) \\
111011\_H\_G & 55\,846&690 & 26&6(1) & .&. & .&. & .&. & .&. & 32&5(14) & 35&2(11) & .&. \\
111011\_H\_R & 55\,846&703 & 22&2(1) & .&. & .&. & 24&7(8) & .&. & .&. & .&. & .&. \\
111011\_H\_V & 55\,846&703 & 26&8(1) & 18&9(45) & 17&1(5) & .&. & .&. & 33&9(20) & 34&7(28) & .&. \\
131207\_C & 56\,634&262 & -70&0(1) & -93&6(27) & -76&2(4) & -72&4(8) & -78&4(36) & -80&0(15) & -67&4(22) & -66&7(34) \\
131209\_C & 56\,636&262 & 19&0(1) & 9&1(46) & 11&2(5) & 18&8(8) & 17&0(49) & 26&4(18) & 33&7(23) & 14&0(32) \\
140515\_C & 56\,793&547 & 60&8(1) & 64&8(56) & 49&8(7) & 61&1(12) & 51&0(93) & 74&5(26) & 68&0(33) & 64&2(58) \\
150720\_C & 57\,224&413 & 36&4(1) & 10&2(49) & 26&1(6) & 39&1(9) & 41&9(40) & 48&6(19) & 55&9(22) & 27&6(43) \\
160325\_C & 57\,473&679 & -49&4(1) & -63&7(56) & -58&0(10) & -52&9(16) & .&. & -45&3(29) & -37&1(56) & .&. \\
160707\_M & 57\,577&412 & 56&0(1) & 43&3(29) & 45&4(4) & 60&6(5) & 47&6(34) & 56&9(11) & 60&7(23) & 60&4(30) \\
181125\_I & 58\,448&293 & -70&0(1) & -86&3(25) & -77&7(4) & -77&5(4) & -65&5(26) & -67&6(13) & -59&0(14) & -75&7(24) \\
181127\_I & 58\,450&307 & 0&8(1) & -5&3(38) & -10&7(6) & -0&6(6) & -1&0(30) & 8&8(15) & 10&6(17) & -8&2(30) \\
190707\_I & 58\,672&553 & -70&0(1) & -89&2(21) & -77&7(4) & -77&5(4) & -65&4(26) & -69&7(10) & -61&6(13) & -77&1(21) \\
190709\_I & 58\,674&504 & 16&8(1) & 5&9(30) & 8&3(5) & 16&7(5) & 28&0(32) & 27&6(11) & 27&4(13) & 13&8(16) \\
191015\_I & 58\,772&371 & -9&8(1) & -16&7(35) & -13&9(5) & -11&4(6) & -7&0(35) & -5&8(15) & -2&5(20) & -17&1(24) \\
\hline  RV mean & .&. & 15&3 & -6&9 & -0&9 & 7&3 & 16&8 & 18&4 & 21&3 & 3&6 \\
$\sigma$ RV & .&. & 43&1 & 48&9 & 43&5 & 47&0 & 38&6 & 48&3 & 45&1 & 46&2 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4388}, 4471, 4713, 4922, 5876, 6678, \HeII{4542}, 5412, and H$\gamma$+\HeII{4338}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{landscape}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for BD~+36\,4063]{Radial velocity measurements for BD~+36\,4063. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:BD+364063}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\SiIII{4553}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
180919\_I & 58\,381&533 & 81&6(1) & 59&4(14) & 60&8(12) & 72&3(9) & 82&3(45) & 89&5(21) & 63&3(34) \\
181125\_I & 58\,448&388 & 155&6(2) & 138&9(10) & 134&4(9) & 141&9(8) & 157&6(37) & 156&5(16) & 150&4(22) \\
181127\_I & 58\,450&429 & -157&8(2) & -171&0(18) & -186&7(10) & -168&5(9) & -164&7(75) & -156&6(26) & -180&7(40) \\
190705\_I & 58\,670&588 & 19&8(1) & 1&5(9) & 2&2(10) & 7&6(7) & 19&2(42) & 19&5(13) & 1&3(21) \\
190707\_I & 58\,672&599 & -94&4(2) & -112&0(8) & -106&3(8) & -110&0(7) & -74&9(57) & -80&9(21) & -120&9(15) \\
190714\_I & 58\,679&448 & 158&0(3) & 136&7(12) & 141&3(7) & 150&8(6) & 127&5(48) & 156&2(17) & 138&6(21) \\
190831\_I & 58\,727&473 & 171&2(4) & 157&7(13) & 152&9(10) & 156&7(8) & 348&1(63) & 159&7(19) & 173&1(37) \\
191012\_I & 58\,769&423 & 7&4(1) & -10&3(9) & -8&6(10) & 2&0(8) & 7&1(64) & 8&2(17) & -1&5(15) \\
191014\_I & 58\,771&405 & 64&0(2) & 49&2(11) & 47&0(13) & 55&8(10) & 63&0(55) & 63&3(18) & 54&1(20) \\
\hline  RV mean & .&. & 45&0 & 27&8 & 26&3 & 34&3 & 62&8 & 46&2 & 30&9 \\
$\sigma$ RV & .&. & 108&1 & 107&4 & 109&2 & 108&4 & 137&7 & 104&8 & 114&2 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4144}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HDE~229\,234]{Radial velocity measurements for HDE~229\,234. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HDE229234}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{4713}} & \multicolumn{2}{c}{\HeI{4922}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{4686}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} & \multicolumn{2}{c}{\SiIII{4553}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
130821\_C & 56\,526&395 & 29&0(1) & 20&8(22) & 25&5(17) & 36&6(26) & 39&7(22) & 27&9(5) & 33&8(15) & 23&7(42) & 38&3(26) & 33&8(17) & 37&6(17) & 38&2(82) \\
130823\_C & 56\,528&606 & -64&2(1) & -70&2(17) & -71&2(14) & -60&5(18) & -58&2(14) & -63&9(4) & -61&7(11) & -64&1(32) & -48&7(18) & -58&1(11) & -53&9(11) & -70&2(53) \\
131208\_C & 56\,635&272 & 29&6(1) & 29&2(18) & 24&3(12) & 31&5(17) & 35&2(12) & 30&2(3) & 35&4(11) & 32&8(31) & 42&2(15) & 42&0(14) & 35&7(11) & 36&5(60) \\
150830\_C & 57\,265&504 & -70&0(1) & -70&5(36) & -77&1(25) & -56&9(41) & -65&3(25) & -67&6(7) & -70&3(13) & -60&8(63) & -66&1(29) & -66&9(21) & -64&6(23) & .&. \\
181127\_I & 58\,450&298 & 22&6(1) & 27&2(15) & .&. & 25&0(16) & 25&4(10) & 22&4(4) & 30&8(6) & 26&0(21) & 34&4(10) & 29&9(10) & 30&5(10) & 23&3(49) \\
190706\_I & 58\,671&600 & 18&8(1) & 20&4(12) & .&. & 20&5(11) & 22&8(7) & 19&1(3) & 25&9(5) & 25&4(14) & 27&0(9) & 25&2(7) & 28&2(7) & 13&6(34) \\
190708\_I & 58\,673&626 & -66&0(1) & -70&3(10) & .&. & -63&6(10) & -60&8(7) & -65&6(3) & -65&8(4) & -62&8(16) & -56&8(8) & -60&1(7) & -59&8(7) & -74&1(34) \\
190713\_I & 58\,678&513 & 15&2(1) & 17&7(10) & .&. & 20&8(13) & 21&0(8) & 14&6(3) & 21&3(6) & 24&9(15) & 23&4(10) & 29&3(9) & 27&5(10) & 14&3(37) \\
190902\_I & 58\,729&555 & -77&2(1) & -71&7(13) & .&. & -76&0(16) & -69&9(11) & -78&1(4) & -77&6(7) & -77&2(22) & -65&6(11) & -72&5(10) & -68&4(10) & -94&1(49) \\
191014\_I & 58\,771&425 & -75&2(1) & -74&0(13) & .&. & -71&1(13) & -69&7(10) & -74&6(3) & -73&9(7) & -70&8(19) & -67&8(10) & -70&4(10) & -68&8(8) & -70&0(45) \\
\hline RV mean & .&. & -23&7 & -24&1 & -24&6 & -19&4 & -18&0 & -23&6 & -20&2 & -20&3 & -14&0 & -16&8 & -15&6 & -20&3 \\
$\sigma$ RV & .&. & 47&1 & 47&3 & 49&6 & 46&7 & 47&2 & 46&7 & 49&9 & 47&1 & 47&6 & 49&1 & 47&8 & 51&9 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4388}, 4471, 4713, 4922, 5016, 5876, \HeII{4200}, 5412 and H$\gamma$+\HeII{4338}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\end{landscape}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~192\,281]{Radial velocity measurements for HD~192\,281. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD192281}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{4686}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
000707\_P       & 51\,733&604 & -28&8(1) & -37&5(31) & -26&1(29) & -49&2(28) & -27&0(17) & .&. \\
000912\_P       & 51\,800&344 & -31&6(1) & -48&7(37) & -26&4(28) & -53&0(27) & -30&2(15) & .&. \\
040828\_P       & 53\,246&417 & -32&2(1) & -62&5(26) & -23&7(18) & -46&6(16) & -24&7(16) & .&. \\
050817\_P       & 53\,600&453 & -24&8(1) & -34&9(30) & -28&0(37) & -46&0(34) & -29&5(17) & 47&4(93) \\
100807\_I       & 55\,416&728 & -27&6(1) & -38&1(15) & -27&9(9) & -69&0(14) & -22&4(8) & -8&8(30) \\
101024\_I       & 55\,494&318 & -22&2(1) & -29&9(13) & -23&4(9) & -43&9(12) & -18&0(7) & -1&4(33) \\
110910\_I       & 55\,815&492 & -18&8(1) & -22&8(15) & -22&8(11) & -43&3(15) & -9&2(8) & -6&6(36) \\
111108\_M       & 55\,874&389 & -31&0(1) & -36&6(15) & -27&4(12) & -57&6(13) & -28&7(8) & 1&5(60) \\
131208\_C       & 56\,635&382 & -34&8(1) & -48&6(25) & -42&8(35) & -30&5(32) & -44&8(16) & .&. \\
140606\_C       & 56\,815&647 & -34&0(1) & -57&1(25) & -36&1(25) & -62&7(27) & -32&6(14) & .&. \\
140706\_C       & 56\,845&551 & -32&4(1) & -45&3(35) & -44&8(53) & -27&7(43) & -27&2(22) & .&. \\
150901\_P       & 57\,267&400 & -29&2(1) & -50&0(11) & -29&6(8) & -56&0(9) & -17&4(6) & -14&7(29) \\
180327\_C\_V    & 58\,205&626 & -33&0(1) & -41&4(18) & .&. & .&. & -27&0(14) & .&. \\
180327\_C\_V\_2 & 58\,205&670 & -20&0(1) & -36&8(18) & .&. & .&. & -10&9(16) & .&. \\
180328\_C\_V    & 58\,206&134 & .&. & -43&7(23) & .&. & .&. & .&. & .&. \\
180328\_C\_V\_2 & 58\,206&710 & -34&2(1) & -43&9(18) & .&. & .&. & -27&3(14) & .&. \\
180404\_C\_V    & 58\,213&656 & -31&2(1) & -37&5(22) & .&. & .&. & -27&6(17) & .&. \\
190901\_I       & 58\,728&585 & -24&4(1) & -36&6(26) & -23&7(28) & -21&6(26) & -23&7(16) & -63&0(102) \\
\hline  RV mean & .&. & -28&8 & -40&6 & -28&2 & -46&7 & -26&0 & -6&0 \\
$\sigma$ RV & .&. & 4&9 & 7&9 & 5&6 & 13&2 & 4&2 & 5&7 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{5876}, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HDE~229\,232~AB]{Radial velocity measurements for HDE~229\,232~AB. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HDE229232AB}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
131208\_C & 56\,635&321 & -18&2(1) & -39&5(28) & -62&7(52) & -7&0(18) \\
161028\_I & 57\,690&387 & -38&0(1) & -32&8(16) & -44&2(23) & -33&7(9) \\
181125\_I & 58\,448&310 & -15&4(1) & -30&3(16) & -26&6(22) & -9&6(10) \\
181128\_I & 58\,451&401 & -29&6(1) & -51&5(19) & -38&6(24) & -21&8(11) \\
190706\_I & 58\,671&669 & -30&2(1) & -54&1(16) & -32&0(19) & -21&6(9) \\
190709\_I & 58\,674&561 & -17&0(1) & -38&4(18) & -17&5(22) & -7&3(10) \\
190713\_I & 58\,678&535 & -47&6(1) & -54&4(14) & -58&6(20) & -35&4(10) \\
190831\_I & 58\,727&629 & -18&0(1) & -14&3(15) & -66&4(27) & -3&1(12) \\
191014\_I & 58\,771&446 & -16&2(1) & -33&4(22) & -23&2(25) & -9&5(13) \\
\hline  RV mean & .&. & -20&7 & -38&7 & -41&1 & -16&6 \\
$\sigma$ RV & .&. & 5&9 & 12&4 & 17&0 & 11&3 \\
Drop & .&. & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4471}, 5876, \HeII{4200}, 4542, 5412, 6527, 6560, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for ALS~15\,133]{Radial velocity measurements for ALS~15\,133. Errors in parenthesis corresponds to the last digit.\\ \label{rvt:ALS15133}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{6678}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
181128\_I & 58\,451&435 & -6&6(6) & -6&6(7) & -4&8(7) & -2&2(34) & -4&6(19) \\
\hline  RV mean & .&. & -6&6 & -6&6 & -4&8 & -2&2 & -4&6 \\
$\sigma$ RV & .&. & 0&0 & 0&0 & 0&0 & 0&0 & 0&0 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for Cyg~OB2-A11]{Radial velocity measurements for Cyg~OB2-A11. Errors in parenthesis corresponds to the last digit.\\ \label{rvt:CygOB2-A11}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\HeII{8237}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
120421\_H\_R & 56\,039&924 & .&. & .&. & -7&0(23) & .&. & .&. & .&. \\
120421\_H\_V & 56\,039&924 & -0&6(20) & -10&2(11) & .&. & 4&5(20) & .&. & 11&7(32) \\
120423\_H\_G & 56\,041&416 & .&. & .&. & .&. & -20&6(19) & .&. & -12&0(32) \\
121210\_H\_R & 56\,272&545 & .&. & .&. & -12&2(25) & .&. & .&. & .&. \\
121210\_H\_V & 56\,272&545 & -12&8(18) & -16&1(11) & .&. & -4&0(22) & .&. & -4&5(28) \\
121211\_H\_R & 56\,273&551 & .&. & .&. & -24&9(30) & .&. & .&. & .&. \\
121211\_H\_V & 56\,273&551 & -34&2(19) & -28&1(14) & .&. & -23&0(24) & .&. & -20&9(30) \\
161019\_M    & 57\,681&475 & -36&7(59) & -44&4(57) & -49&6(32) & .&. & -39&8(30) & 30&7(26.1) \\
161019\_M\_2 & 57\,681&496 & -54&1(100) & -41&3(57) & -30&3(39) & .&. & -27&3(32) & .&. \\
181129\_I    & 58\,452&326 & -36&0(39) & -40&3(32) & -62&5(24) & -58&4(81) & -35&6(34) & -33&1(95) \\
190709\_I    & 58\,674&595 & 1&1(19) & -13&7(13) & 3&0(18) & 10&9(30) & 15&2(19) & 5&5(23) \\
191012\_I    & 58\,769&482 & 8&0(31) & -7&3(20) & 19&0(23) & 18&8(44) & 24&0(31) & 21&9(41) \\
\hline  RV mean & .&. & -20&7 & -25&2 & -20&6 & -10&3 & -12&7 & -0&1 \\
$\sigma$ RV & .&. & 21&1 & 14&3 & 25&2 & 24&3 & 26&8 & 20&3 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for Cyg~OB2-22~C.  Errors in parenthesis corresponds to the last digit.\\ \label{rvt:CygOB2-22C}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{5412}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
120412\_H\_V & 56\,031&460 & 4&0(46) & 30&5(145) \\
120422\_H\_V & 56\,041&430 & -16&3(27) & 35&6(91) \\
120605\_H\_G & 56\,085&297 & .&. & 22&5(94) \\
\hline  RV mean & .&. & -6&2 & 29&4 \\
$\sigma$ RV & .&. & 10&2 & 5&4 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for Cyg~OB2-41.  Errors in parenthesis corresponds to the last digit.\\ \label{rvt:CygOB2-41}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
190714\_I & 58\,679&588 & -42&3(71) & -42&0(59) \\
191015\_I & 58\,772&473 & -42&2(43) & -24&6(46) \\
\hline  RV mean & .&. & -42&2 & -33&3 \\
$\sigma$ RV & .&. & 0&0 & 8&7 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for ALS~15\,148]{Radial velocity measurements for ALS~15\,148. Errors in parenthesis corresponds to the last digit.\\ 
\label{rvt:ALS15148}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
120522\_H\_R & 56\,070&850 & .&. & .&. & .&. & -60&4(50) & .&. & .&. \\
120522\_H\_V & 56\,070&850 & -39&6(1) & -57&4(41) & -36&1(23) & .&. & -39&6(41) & -21&4(79) \\
120620\_H\_B & 56\,099&763 & -34&6(1) & .&. & .&. & .&. & .&. & .&. \\
120620\_H\_G & 56\,099&763 & -30&2(1) & .&. & .&. & .&. & -28&7(20) & -5&0(37) \\
121212\_H\_R & 56\,274&549 & .&. & .&. & .&. & -5&7(52) & .&. & .&. \\
121212\_H\_V & 56\,274&549 & -8&4(1) & -38&2(37) & -7&4(22) & .&. & -3&3(30) & 7&4(63) \\
190705\_I & 58\,670&553 & -43&4(1) & -40&3(40) & -36&0(22) & -29&6(27) & -32&0(41) & -48&4(66) \\
190707\_I & 58\,672&640 & 17&8(1) & -2&5(44) & 23&3(20) & 14&9(29) & 30&8(42) & 42&6(51) \\
190713\_I & 58\,678&593 & 33&4(1) & -7&7(44) & 27&3(20) & 34&8(31) & 38&1(41) & 41&7(54) \\
191015\_I & 58\,772&443 & -37&6(1) & -59&4(82) & -41&4(44) & -25&1(53) & -46&5(71) & .&. \\
\hline  RV mean & .&. & -32&3 & -34&2 & -11&7 & -11&8 & -11&6 & 2&8 \\
$\sigma$ RV & .&. & 11&4 & 22&1 & 28&4 & 31&0 & 31&7 & 32&6 \\
Drop & .&. & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4144}, 4388, 4471, 5016, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for Cyg~OB2-1. Errors in parenthesis corresponds to the last digit.\\  \label{rvt:CygOB2-1}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
181128\_I & 58\,451&340 & 6&4(30) & 27&1(8) & 30&0(43) & 60&0(21) \\
191014\_I & 58\,771&497 & 25&9(47) & 41&0(12) & 48&4(62) & 58&6(33) \\
\hline  RV mean & .&. & 16&2 & 34&0 & 39&2 & 59&3 \\
$\sigma$ RV & .&. & 9&8 & 7&0 & 9&2 & 0&7 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for ALS~15\,131. Errors in parenthesis corresponds to the last digit.\\  \label{rvt:ALS15131}}
\begin{tabular}{l r@{.}l  r@{.}l  }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\HeI{5876}}  \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
190902\_I & 58\,729&453 &  -2&4(14) \\
\hline  RV mean & .&. & -2&4 \\
$\sigma$ RV & .&. & 0&0 \\
Drop & .&. &  \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for Cyg~OB2-20. Errors in parenthesis corresponds to the last digit.\\  \label{rvt:CygOB2-20}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{6678}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} & \multicolumn{2}{c}{\SiIII{4553}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
181129\_I & 58\,452&370 & -33&9(37) & -24&6(20) & -26&6(4) & -31&2(5) & -27&2(34) & -25&5(16) & -32&6(16) \\
190713\_I & 58\,678&647 & -24&9(17) & -26&9(8) & -24&9(2) & -28&8(2) & -25&8(15) & -26&9(5) & -31&8(8) \\
190901\_I & 58\,728&466 & -29&7(20) & -28&8(15) & -28&8(5) & -33&2(3) & -17&1(28) & -31&6(7) & -34&3(11) \\
\hline  RV mean & .&. & -29&5 & -26&8 & -26&8 & -31&1 & -26&5 & -28&0 & -32&9 \\
$\sigma$ RV & .&. & 3&7 & 1&7 & 1&6 & 1&8 & 0&7 & 2&6 & 1&0 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for Cyg~OB2-15. Errors in parenthesis corresponds to the last digit.\\  \label{rvt:CygOB2-15}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{6678}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
190705\_I & 58\,670&647 & 0&8(24) & -6&1(23) & 10&7(7) & 29&3(14) & 25&7(37) & 25&4(14) & 30&6(23) \\
190709\_I & 58\,674&640 & -80&5(26) & -57&9(21) & -47&3(7) & -14&9(13) & -46&6(31) & -41&6(14) & -37&0(25) \\
190901\_I & 58\,728&516 & 76&3(37) & 38&9(66) & 26&0(9) & 54&2(24) & .&. & 42&1(21) & 29&1(30) \\
191015\_I & 58\,772&504 & 2&5(62) & 7&3(45) & 23&4(12) & 46&0(25) & 36&5(73) & 44&2(25) & 44&6(42) \\
\hline  RV mean & .&. & -0&2 & -4&4 & 20&0 & 28&6 & 31&1 & 37&2 & 34&8 \\
$\sigma$ RV & .&. & 55&5 & 34&9 & 6&7 & 26&7 & 5&4 & 8&4 & 7&0 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for Cyg~OB2-11]{Radial velocity measurements for Cyg~OB2-11. Errors in parenthesis corresponds to the last digit.\\ 
\label{rvt:CygOB2-11}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
110517\_H\_B & 55\,699&866 & -26&4(1) & .&. & -38&9(15) & .&. & -27&0(8) & .&. \\
110517\_H\_G & 55\,699&866 & -27&4(1) & .&. & .&. & .&. & .&. & -25&8(8) \\
110517\_H\_V & 55\,699&886 & -40&0(1) & -48&1(14) & .&. & -40&3(13) & .&. & -24&8(21) \\
160428\_I & 57\,507&654 & -26&6(1) & -46&3(7) & -29&2(28) & -37&4(7) & -29&1(16) & -26&0(10) \\
190708\_I & 58\,673&713 & -29&4(1) & -50&5(8) & -44&0(24) & -40&1(9) & -26&9(15) & -27&8(9) \\
\hline  RV mean & .&. & -27&4 & -48&3 & -37&4 & -40&2 & -27&0 & -26&1 \\
$\sigma$ RV & .&. & 1&2 & 1&7 & 6&1 & 0&1 & 0&1 & 1&1 \\
Drop & .&. & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4471}, 5016, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for 68~Cyg]{Radial velocity measurements for 68~Cyg. Errors in parenthesis corresponds to the last digit.\\ 
\label{rvt:68Cyg}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
081108\_I & 54\,779&430 & 10&6(1) & 5&2(13) & 17&5(12) & 9&9(8) & 21&9(19) \\
110613\_M & 55\,726&610 & 36&0(1) & 27&7(12) & 51&3(14) & 51&2(9) & 61&6(22) \\
110615\_M & 55\,728&701 & 37&6(1) & 32&5(9) & 49&3(10) & 50&3(7) & 54&6(17) \\
110617\_M & 55\,730&509 & 33&2(1) & 20&3(11) & 49&5(12) & 51&6(9) & 54&9(21) \\
110617\_M\_2 & 55\,730&565 & 32&0(1) & 20&3(12) & 44&5(12) & 50&3(9) & 61&2(21) \\
110617\_M\_3 & 55\,730&622 & 35&0(1) & 24&8(10) & 44&6(12) & 51&8(8) & 64&2(20) \\
110617\_M\_4 & 55\,730&669 & 40&2(1) & 30&7(10) & 51&7(13) & 57&0(7) & 61&9(21) \\
110617\_M\_5 & 55\,730&737 & 39&4(1) & 32&3(7) & 50&8(12) & 54&0(7) & 55&8(20) \\
110618\_M & 55\,731&530 & 39&0(1) & 30&5(11) & 50&3(18) & 52&6(9) & 66&1(27) \\
110618\_M\_2 & 55\,731&586 & 37&2(1) & 29&5(11) & 50&1(13) & 52&8(8) & 58&1(22) \\
110618\_M\_3 & 55\,731&640 & 35&8(1) & 25&6(10) & 50&7(13) & 51&3(7) & 59&6(19) \\
110618\_M\_4 & 55\,731&693 & 36&4(1) & 26&5(10) & 51&2(12) & 52&3(8) & 61&1(20) \\
110619\_M & 55\,732&517 & 41&2(1) & 35&4(10) & 52&3(12) & 58&5(8) & 66&1(20) \\
110619\_M\_2 & 55\,732&575 & 41&2(1) & 34&6(11) & 52&8(12) & 56&7(8) & 68&3(20) \\
110619\_M\_3 & 55\,732&614 & 38&8(1) & 29&9(10) & 49&0(11) & 53&6(8) & 61&6(20) \\
110619\_M\_4 & 55\,732&665 & 39&0(1) & 32&3(9) & 52&8(11) & 53&0(7) & 55&5(18) \\
110619\_M\_5 & 55\,732&719 & 35&8(1) & 26&8(10) & 51&3(12) & 51&2(8) & 61&0(21) \\
110620\_M & 55\,733&493 & 37&0(1) & 26&9(9) & 48&5(13) & 49&3(8) & 58&0(20) \\
121223\_I & 56\,285&318 & 28&6(1) & 14&5(9) & 46&0(13) & 40&6(8) & 45&5(22) \\
130817\_C & 56\,522&677 & 21&8(1) & 12&4(16) & 9&0(29) & 38&7(17) & 37&0(38) \\
140607\_C & 56\,816&602 & 2&0(1) & -14&7(14) & -2&4(25) & 5&3(14) & 4&9(39) \\
140705\_C & 56\,844&582 & 1&8(1) & -10&2(14) & -2&3(25) & 6&1(14) & 5&9(37) \\
140707\_C & 56\,846&649 & 5&8(1) & -6&3(16) & 0&3(33) & 6&2(17) & 6&9(47) \\
150528\_M & 57\,171&677 & 16&2(1) & 7&5(10) & 15&7(17) & 20&7(9) & 28&4(26) \\
150529\_M & 57\,172&734 & 16&0(1) & 5&1(10) & 15&6(16) & 17&4(10) & 30&6(28) \\
150530\_M & 57\,173&748 & 14&8(1) & 3&5(10) & 27&5(50) & 13&7(17) & 15&7(45) \\
160718\_C & 57\,588&551 & 4&0(1) & -2&7(17) & -10&7(26) & 19&9(13) & 28&0(32) \\
171008\_I & 58\,035&373 & 17&8(1) & 3&2(12) & 18&2(15) & 18&1(9) & 14&5(21) \\
171120\_M & 58\,078&306 & 4&8(1) & -14&0(8) & 4&8(10) & 7&6(6) & 42&1(22) \\
171121\_M & 58\,079&334 & 12&0(1) & -4&6(10) & 5&7(13) & 15&3(7) & 48&3(21) \\
190831\_I & 58\,727&668 & 35&0(1) & 14&7(13) & 52&6(18) & 52&3(11) & -20&5(36) \\
190901\_I & 58\,728&354 & 29&6(1) & 9&5(17) & 54&3(18) & 34&7(16) & 23&7(50) \\
961126\_P & 50\,414&237 & 5&4(1) & -9&7(16) & 15&8(19) & 9&1(12) & 8&8(34) \\
\hline  RV mean & .&. & 30&1 & 15&2 & 50&2 & 49&3 & 43&5 \\
$\sigma$ RV & .&. & 10&6 & 15&7 & 2&6 & 8&4 & 20&8 \\
Drop & .&. & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{13} & \multicolumn{2}{c}{11} & \multicolumn{2}{c}{1} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4121}, 4144, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Radial velocity measurements for HD~108. Errors in parenthesis corresponds to the last digit.\\ \label{rvt:HD108}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
001210\_P    & 51\,889&370 & -65&4(9) & -73&7(14) & -81&0(8) & -76&6(8) \\
010811\_P    & 52\,133&589 & -61&9(7) & -71&9(11) & -75&9(6) & -73&6(7) \\
041116\_P    & 53\,326&336 & -55&1(7) & -65&5(11) & -69&6(6) & -64&3(12) \\
050816\_P    & 53\,599&622 & -54&6(11) & -65&4(28) & -69&0(7) & -64&1(10) \\
100908\_I    & 55\,448&472 & -59&6(3) & -70&2(5) & -75&7(4) & -71&5(3) \\
101113\_P    & 55\,514&246 & -59&3(4) & -73&4(6) & -80&3(4) & -73&4(5) \\
101113\_P\_2 & 55\,514&252 & -59&3(3) & -73&4(6) & -79&7(5) & -74&9(5) \\
101113\_P\_3 & 55\,514&258 & -58&7(4) & -73&6(6) & -80&1(4) & -73&4(5) \\
101113\_P\_4 & 55\,514&265 & -59&9(3) & -73&4(6) & -80&2(4) & -71&9(5) \\
101113\_P\_5 & 55\,514&271 & -59&3(3) & -72&3(6) & -79&6(4) & -71&4(5) \\
110714\_H\_B & 55\,757&962 & .&. & -68&1(10) & .&. & .&. \\
110714\_H\_G & 55\,757&962 & .&. & .&. & -74&4(6) & -68&9(8) \\
110718\_H\_V & 55\,761&938 & -55&6(9) & .&. & -72&3(7) & -69&2(11) \\
110909\_I    & 55\,814&562 & -55&5(3) & -68&3(6) & -72&5(4) & -69&6(4) \\
110930\_H\_B & 55\,835&844 & .&. & -69&8(10) & .&. & .&. \\
110930\_H\_G & 55\,835&844 & .&. & .&. & -73&7(6) & -69&0(5) \\
110930\_H\_V & 55\,835&847 & -56&4(6) & .&. & -73&0(6) & -68&6(8) \\
121223\_I    & 56\,285&420 & -54&8(5) & -66&1(8) & -70&1(4) & -66&4(5) \\
121223\_I\_2 & 56\,285&430 & -53&9(4) & -63&7(6) & -70&3(4) & -67&0(4) \\
130129\_I    & 56\,322&337 & -54&1(3) & -63&3(5) & -69&4(4) & -66&8(3) \\
131207\_C    & 56\,634&497 & -52&5(8) & -68&8(14) & -68&8(6) & -64&7(9) \\
140905\_C    & 56\,906&690 & -51&5(9) & -62&9(13) & -68&7(7) & -63&6(10) \\
150105\_C    & 57\,028&300 & -51&7(13) & -67&8(22) & -70&5(10) & -69&1(16) \\
150113\_C    & 57\,036&342 & -56&5(15) & -70&3(24) & -70&3(11) & -68&8(21) \\
150830\_C    & 57\,265&582 & -56&3(13) & -70&1(18) & -73&0(10) & -70&2(14) \\
150901\_P    & 57\,267&517 & -57&0(4) & -69&5(6) & -72&3(4) & -70&1(4) \\
160721\_C    & 57\,591&635 & -65&6(11) & -84&9(21) & -81&2(8) & -79&3(13) \\
161017\_M    & 57\,679&347 & -65&6(5) & -76&8(9) & -82&0(4) & -77&3(7) \\
161018\_M    & 57\,680&611 & -64&9(6) & -76&3(8) & -82&4(4) & -77&5(5) \\
161020\_M    & 57\,682&697 & -63&1(4) & -75&6(8) & -81&4(4) & -77&8(6) \\
171027\_M    & 58\,054&486 & -63&4(5) & -75&9(9) & -80&5(5) & -74&7(7) \\
180530\_S    & 58\,269&677 & -61&1(8) & -71&9(21) & -79&9(11) & -77&7(16) \\
181020\_M    & 58\,412&576 & -61&8(2) & -73&2(5) & -78&9(3) & -74&5(3) \\
181127\_I    & 58\,450&542 & -62&1(3) & -74&7(7) & -77&9(3) & -74&4(3) \\
190922\_C\_V & 58\,749&492 & -59&6(4) & .&. & -77&8(7) & -73&4(7) \\
\hline  RV mean & .&. & -58&6 & -70&5 & -75&5 & -71&3 \\
$\sigma$ RV & .&. & 4&1 & 4&0 & 4&7 & 4&3 \\
Drop & .&. & \multicolumn{2}{c}{0} & 1&0 & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for V747~Cep]{Radial velocity measurements for V747~Cep. Errors in parenthesis corresponds to the last digit.\\ 
\label{rvt:V747Cep}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{H{$\alpha$}} & \multicolumn{2}{c}{H{$\beta$}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{4686}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
111001\_H\_B & 55\,836&730 & -11&4(1)  & .&. & .&. & .&. & .&. & -7&5(14) & -22&4(14) & .&. & .&. \\
111001\_H\_G & 55\,836&730 & -11&0(1)  & .&. & .&. & -31&7(5) & .&. & .&. & .&. & -3&7(16) & -36&4(33) \\
111001\_H\_R & 55\,836&774 & -10&2(1)  & .&. & -35&6(15) & .&. & .&. & .&. & .&. & .&. & .&. \\
111001\_H\_V & 55\,836&774 & -9&4(1)   & -27&6(51) & .&. & .&. & -9&9(26) & .&. & .&. & 3&7(27) & -48&9(97) \\
120908\_C    & 56\,179&636 & 27&8(1)   & 12&2(46) & -7&9(10) & 12&4(13) & 27&5(22) & .&. & 20&4(32) & 53&6(19) & 7&5(42) \\
121205\_C    & 56\,267&531 & -150&2(1) & -155&9(41) & -190&6(12) & -167&1(38) & -154&6(29) & .&. & .&. & -142&8(38) & .&. \\
121230\_C    & 56\,292&431 & 8&8(1)    & -19&4(55) & -14&1(10) & -14&2(23) & 5&3(22) & .&. & 13&1(61) & 35&4(24) & -1&5(61) \\
130201\_C    & 56\,325&289 & -37&0(1)  & -68&0(49) & -57&4(13) & -58&3(22) & -31&9(25) & -37&3(89) & -35&3(47) & -28&5(32) & -41&3(83) \\
130226\_C    & 56\,350&312 & 19&6(1)   & -8&5(79) & 0&2(15) & -4&8(30) & 36&5(31) & 78&0(114) & 45&3(75) & 46&8(31) & 10&8(73) \\
130816\_C    & 56\,521&603 & 23&2(1)   & 5&6(49) & -9&9(10) & 11&3(19) & .&. & -3&3(68) & 24&2(54) & 43&8(26) & 6&5(76) \\
130821\_C    & 56\,526&646 & 35&0(1)   & 2&4(54) & 2&6(11) & 24&6(18) & 29&7(23) & -17&9(95) & 61&6(53) & .&. & 9&4(50) \\
140109\_C    & 56\,667&301 & -132&4(1) & -146&2(37) & -158&8(12) & -146&1(20) & -142&9(25) & -161&4(78) & -116&4(43) & -149&6(22) & -142&8(87) \\   
171001\_I    & 58\,028&467 & -0&0(1)   & -3&1(38) & -29&1(8) & -14&0(15) & -15&6(20) & 22&2(41) & 6&1(28) & 16&3(20) & -21&5(52) \\
171002\_I    & 58\,029&601 & 33&6(1)   & 4&6(47) & 7&0(8) & 16&4(12) & 18&9(21) & 45&9(36) & 37&3(25) & 61&1(18) & 11&4(41) \\
171003\_I    & 58\,030&539 & 24&2(1)   & 20&3(40) & -0&5(7) & 7&7(12) & 6&9(21) & 34&8(32) & 28&6(23) & 43&8(18) & -0&2(35) \\
171119\_I    & 58\,077&539 & 32&2(1)   & 23&0(47) & 1&7(9) & 15&9(14) & 22&8(21) & 41&7(39) & 32&2(28) & 59&0(19) & 18&3(42) \\
180921\_I    & 58\,383&538 & -25&6(1)  & -43&9(21) & -52&2(5) & -41&3(11) & -26&9(12) & -28&6(36) & -37&7(24) & -18&0(16) & -59&9(34) \\
181029\_M    & 58\,421&601 & -128&6(1) & -127&8(19) & -164&0(7) & -144&8(10) & -142&7(15) & -129&2(33) & -147&4(20) & -132&8(12) & -135&0(49) \\
190901\_I    & 58\,728&618 & 28&2(1)   & 50&0(34) & -5&4(8) & 18&0(14) & 26&0(16) & 13&5(59) & 33&0(23) & 36&2(19) & -3&9(45) \\
191014\_I    & 58\,771&550 & 20&8(1)   & 27&4(42) & -6&9(7) & 4&2(14) & 11&8(19) & 25&5(37) & 23&9(24) & 40&9(20) & -8&2(46) \\
\hline  RV mean & .&. & 8&8 & -1&8 & -14&8 & -3&8 & 7&8 & -3&3 & 16&5 & 27&9 & -10&5 \\
$\sigma$ RV & .&. & 21&9 & 29&4 & 19&9 & 24&1 & 21&5 & 46&1 & 28&5 & 27&9 & 24&0 \\
Drop & .&. & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{5876}, \HeII{5412}, 6560 and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~12\,323]{Radial velocity measurements for HD~12\,323.  Errors in parenthesis corresponds to the last digit.\\ 
\label{rvt:HD12323}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
041119\_P & 53\,329&273 & -58&8(1) & -69&7(31) & -52&8(13) & .&. & -57&8(75) & -58&9(27) \\
041119\_P\_2 & 53\,329&349 & -65&4(1) & -72&8(32) & -61&0(12) & .&. & -68&6(67) & -70&2(26) \\
041119\_P\_3 & 53\,329&426 & -71&2(1) & -84&1(25) & -67&6(12) & .&. & -75&2(58) & -70&3(23) \\
051105\_P & 53\,680&547 & -37&2(1) & -52&7(78) & -38&5(11) & .&. & .&. & -35&6(27) \\
051110\_P & 53\,685&474 & -64&4(1) & -77&2(18) & -56&7(9) & .&. & -58&3(59) & -70&4(23) \\
051110\_P\_2 & 53\,685&517 & -67&4(1) & -80&3(28) & -58&5(13) & .&. & -55&4(86) & -61&6(30) \\
110911\_I & 55\,816&730 & -70&8(1) & -80&2(6) & -64&1(4) & -59&6(9) & -62&3(21) & -67&7(6) \\
121028\_M & 56\,229&591 & -21&8(1) & -32&8(34) & -21&7(30) & -14&4(44) & .&. & -30&7(57) \\
121028\_M\_2 & 56\,229&624 & -23&4(1) & -35&6(14) & -17&9(10) & -15&7(17) & -9&2(49) & -22&9(22) \\
121225\_I & 56\,287&460 & -18&8(1) & -28&7(6) & -12&6(3) & -7&9(7) & -6&7(23) & -14&4(7) \\
161028\_I & 57\,690&545 & -45&4(1) & -54&5(7) & -37&2(4) & -38&0(6) & -27&1(27) & -39&4(9) \\
190902\_I & 58\,729&645 & -77&0(1) & -86&1(8) & -70&0(5) & -68&7(9) & -70&3(28) & -77&2(13) \\
191012\_I & 58\,769&605 & -50&6(1) & -58&9(8) & -43&7(5) & -39&0(8) & -37&9(29) & -47&8(10) \\
191013\_I & 58\,770&533 & -45&0(1) & -57&4(8) & -39&1(6) & -37&4(10) & -31&6(32) & -41&8(13) \\
201013\_C\_V & 59\,136&565 & -24&4(1) & .&. & -16&8(4) & -15&0(5) & .&. & -21&0(14) \\
201013\_C\_V\_2 & 59\,136&586 & -22&8(1) & .&. & -15&3(4) & -13&3(6) & .&. & -19&9(14) \\
201014\_C\_V & 59\,137&459 & -66&4(1) & .&. & -60&1(7) & -56&0(11) & .&. & -63&8(21) \\
\hline  RV mean & .&. & -48&9 & -62&2 & -43&2 & -33&2 & -46&7 & -47&9 \\
$\sigma$ RV & .&. & 19&9 & 18&8 & 19&5 & 20&4 & 22&6 & 20&5 \\
Drop & .&. & \multicolumn{2}{c}{0}& \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4120}, 4143, 4388, 4471, 4713, 5016, 5048, \HeII{4200}, 4542, 4686, 5412, 6560 and H$\gamma$+\HeII{4338}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{landscape}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~16\,429~Aa]{Radial velocity measurements for HD~16\,429~Aa. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD16429Aa}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5015}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{6678}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} & \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
001215\_P & 51\,894&255 & -35&0(1) & -53&6(47) & -27&4(53) & -36&8(11) & -24&4(51) & .&. & -24&9(48) & -20&3(24) & -13&6(29)           \\
001216\_P & 51\,895&333 & -21&2(1) & -7&1(86) & -13&1(51) & -29&1(10) & -11&4(41) & .&. & -5&3(45) & -5&5(22) & -2&8(26)               \\
011124\_P & 52\,238&370 & -84&8(1) & -107&3(26) & -81&6(59) & -95&1(8) & -76&0(15) & .&. & -86&5(34) & -81&7(19) & -76&2(20)           \\
100908\_I & 55\,448&727 & -69&4(1) & -97&8(14) & -54&4(13) & -74&1(7) & -53&3(11) & -55&6(10) & -87&5(19) & -72&4(13) & -48&3(11)      \\
110905\_H\_B & 55\,810&892 & -31&8(1) & .&. & .&. & .&. & .&. & .&. & -15&2(30) & .&. & .&.                                            \\
110905\_H\_G & 55\,810&892 & -27&4(1) & .&. & -43&7(16) & .&. & .&. & .&. & .&. & -12&1(19) & -11&5(20)                                \\
110906\_H\_R & 55\,811&856 & .&. & .&. & .&. & .&. & -60&7(15) & -77&6(15) & .&. & .&. & .&.                                           \\
110906\_H\_V & 55\,811&856 & -75&2(1) & -93&1(28) & .&. & -79&4(6) & .&. & .&. & .&. & -77&4(17) & -70&1(23)                           \\
110909\_I & 55\,814&623 & -62&0(1) & -73&8(10) & -60&9(9) & -74&2(4) & -64&0(6) & -70&0(6) & -50&0(14) & -52&2(9) & -52&5(7)           \\
111022\_H\_B & 55\,857&712 & -88&2(1) & .&. & .&. & .&. & .&. & .&. & -82&8(19) & .&. & .&.                                            \\
111022\_H\_G & 55\,857&712 & -88&2(1) & .&. & -91&5(10) & .&. & .&. & .&. & .&. & -88&0(11) & -79&1(8)                                 \\
111022\_H\_R & 55\,857&721 & .&. & .&. & .&. & .&. & -93&7(10) & -95&4(13) & .&. & .&. & .&.                                           \\
111022\_H\_V & 55\,857&721 & -96&2(1) & -96&1(22) & .&. & -98&6(6) & .&. & .&. & .&. & -88&2(14) & -83&2(15)                           \\
120910\_C & 56\,181&586 & -51&4(1) & -105&1(28) & -38&9(25) & -50&5(11) & -29&2(14) & -50&4(16) & -63&0(32) & -55&1(23) & -14&6(29)    \\
121023\_C & 56\,224&529 & -73&0(1) & -131&2(46) & -57&6(54) & -71&4(11) & -69&0(30) & -80&2(31) & -69&8(54) & -85&9(38) & -33&0(41)    \\
121121\_C & 56\,253&594 & -15&4(1) & -26&3(43) & -16&3(23) & -19&1(9) & -12&6(15) & -17&6(17) & 10&7(33) & 11&6(16) & 14&2(17)         \\
121205\_C & 56\,267&452 & -59&6(1) & -139&3(38) & -51&0(32) & -58&7(9) & -38&7(24) & -64&5(20) & -57&9(46) & -63&7(30) & -36&1(38)     \\
121223\_I & 56\,285&484 & -65&4(1) & -92&8(17) & -61&1(11) & -72&9(4) & -58&6(8) & -68&6(8) & -63&7(25) & -62&8(13) & -49&2(13)        \\
121228\_C & 56\,290&364 & -2&2(1) & -33&6(30) & -1&6(18) & -3&6(7) & 24&2(16) & 1&6(10) & 14&3(23) & 19&9(12) & 21&3(15)               \\
130130\_C & 56\,323&378 & -32&0(1) & -75&3(33) & -40&5(20) & -34&2(5) & -11&4(23) & -33&7(11) & -14&0(29) & -0&8(16) & -1&8(14)        \\
130201\_C & 56\,325&325 & -82&2(1) & -134&0(40) & -92&4(40) & -83&6(9) & -65&9(20) & -88&9(25) & -57&2(55) & -72&3(26) & -52&4(32)     \\
130925\_C & 56\,561&624 & -66&8(1) & -87&8(42) & -71&1(38) & -82&3(10) & .&. & -102&0(29) & -64&0(42) & -79&8(29) & -52&4(28)          \\
130930\_C & 56\,566&675 & -95&8(1) & -120&5(25) & -103&0(28) & -107&9(6) & -76&1(31) & -106&0(15) & -114&8(40) & -91&3(19) & -89&1(23) \\
131029\_M & 56\,595&553 & -54&0(1) & -70&5(40) & -64&5(24) & -77&8(8) & -62&0(15) & -63&8(14) & -27&6(37) & -27&9(20) & -23&6(27)      \\
140109\_C & 56\,667&340 & -84&6(1) & -112&0(30) & -77&4(28) & -89&5(7) & -79&8(18) & -88&7(15) & -83&2(42) & -102&4(27) & -70&4(25)    \\
140111\_C & 56\,669&338 & -31&0(1) & -53&2(42) & -18&5(31) & -38&3(8) & -26&1(16) & -35&8(17) & -36&2(46) & -14&9(25) & -4&1(24)       \\
140112\_C & 56\,670&374 & -74&6(1) & -101&9(28) & -68&9(23) & -79&8(6) & -61&7(16) & -76&2(15) & -91&4(38) & -78&9(20) & -66&5(24)     \\
181025\_M & 58\,417&634 & -101&2(1) & -112&9(9) & -101&4(7) & -107&0(4) & -91&5(5) & -102&4(5) & -91&7(11) & -99&8(7) & -86&1(8)       \\
191014\_I & 58\,771&580 & -46&4(1) & -104&3(51) & -50&5(29) & -46&6(11) & -29&1(15) & -41&3(16) & -73&7(50) & -48&8(27) & -44&1(28)    \\
\hline  RV mean & .&. & -59&8 & -88&2 & -56&0 & -65&7 & -48&7 & -65&9 & -53&7 & -54&0 & -41&0 \\
$\sigma$ RV & .&. & 27&0 & 34&0 & 27&8 & 27&9 & 29&6 & 28&7 & 34&6 & 36&2 & 32&1 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0}& \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\end{landscape}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~15\,137]{Radial velocity measurements for HD~15\,137. Errors in parenthesis corresponds to the last digit. \\
\label{rvt:HD15137}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l   r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{H{$\alpha$}} & \multicolumn{2}{c}{H{$\beta$}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
041115\_P & 53\,325&451 & -48&6(1) & -72&8(17) & -54&0(11) & -57&2(18) & -4&9(77) & -27&3(54)    & -18&8(57) \\
091112\_I & 55\,148&673 & -53&6(1) & -69&7(9) & -56&0(6) & -60&5(11) & -26&1(31) & -36&4(13)     & -12&7(23) \\
110909\_I & 55\,814&608 & -38&0(1) & -45&7(7) & -40&4(6) & -44&7(10) & -17&9(38) & -11&7(20)     & -30&1(22) \\
121225\_I & 56\,287&436 & -35&6(1) & -55&0(6) & -40&5(5) & -39&9(7) & -3&9(32) & -10&3(15)       & -23&6(23) \\
130226\_C & 56\,350&346 & -44&8(1) & -48&6(11) & -59&8(11) & -41&5(15) & 0&2(86) & -7&0(27)      & -2&5(81) \\
131208\_C & 56\,635&408 & -63&6(1) & -75&4(11) & -63&6(8) & -72&6(11) & -142&5(75) & -52&7(32)   & -65&8(57) \\
140816\_C & 56\,886&671 & -45&0(1) & -62&7(11) & -44&6(9) & -55&8(15) & -36&3(69) & -14&9(31)    & -7&0(66) \\
150819\_C & 57\,254&573 & -50&4(1) & -60&1(12) & -54&2(11) & -57&9(14) & -54&3(85) & -44&6(42)   & -18&1(79) \\
150901\_C & 57\,267&677 & -43&6(1) & -62&0(14) & -45&1(14) & -50&1(17) & -64&9(109) & -26&3(51)  & -10&5(90) \\
160721\_C & 57\,591&602 & -49&0(1) & -47&8(21) & -51&5(15) & -44&4(21) & .&. & -15&1(63)         & .&. \\
170718\_S & 57\,953&623 & -47&2(1) & -57&9(15) & -46&6(15) & -57&4(15) & .&. & -41&2(46)         & .&. \\
171008\_I & 58\,035&653 & -39&2(1) & -53&3(8) & -41&2(6) & -45&6(10) & -30&3(30) & -28&8(9)      & -20&6(22) \\
171120\_M & 58\,078&450 & -66&2(1) & -88&6(5) & -69&8(7) & -70&8(9) & -36&5(42) & -51&1(17)      & -38&4(42) \\
171121\_M & 58\,079&496 & -62&0(1) & -70&2(15) & -65&1(16) & -69&5(21) & -57&9(158) & -60&0(53)  & .&. \\
171221\_M & 58\,109&317 & -52&0(1) & -72&7(6) & -55&8(7) & -56&7(8) & -28&2(28) & -31&1(13)      & -19&8(29) \\
190114\_S & 58\,498&604 & -37&2(1) & -53&5(15) & -35&9(14) & -49&3(21) & -18&5(14.8) & -27&3(44) & .&. \\
190225\_S & 58\,540&453 & -34&4(1) & -47&0(12) & -38&5(10) & -46&4(15) & -4&9(82) & -18&8(33)    & -20&3(69) \\
190314\_S & 58\,557&365 & -38&8(1) & -57&6(12) & -46&3(8) & -49&3(15) & 11&2(59) & -22&4(27)     & -16&5(55) \\
\hline  RV mean & .&. & -47&2 & -61&1 & -50&5 & -53&9 & -24&9 & -29&3  & -18&4 \\
$\sigma$ RV & .&. & 9&3 & 11&4 & 9&6 & 9&7 & 21&8 & 15&2  & 9&0 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5876, \HeII{4200}, 4542, 5412, 6560, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~14\,633~AaAb]{Radial velocity measurements for HD~14\,633~AaAb. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD14633AaAb}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
011121\_P & 52\,235&378 & -35&2(1) & -32&3(7) & .&. & -27&5(31) & -32&2(13) \\
041114\_P & 53\,324&421 & -41&8(1) & -39&8(6) & .&. & -33&7(29) & -39&3(16) \\
091112\_I & 55\,148&632 & -39&0(1) & -33&4(3) & -28&3(5) & -32&3(15) & -34&7(4) \\
110909\_I & 55\,814&579 & -70&2(1) & -69&1(3) & -63&3(5) & -62&5(15) & -66&1(5) \\
121025\_M & 56\,226&559 & -37&0(1) & -33&8(3) & -30&7(5) & -27&0(13) & -33&1(5) \\
121223\_I & 56\,285&471 & -36&4(1) & -33&5(3) & -29&7(4) & -26&5(14) & -32&3(4) \\
130816\_C & 56\,521&655 & -37&6(1) & -32&3(5) & -27&6(12) & -34&0(22) & -34&2(9) \\
140826\_P & 56\,896&651 & -46&6(1) & -43&8(2) & .&. & -34&8(10) & -41&5(4) \\
150105\_C & 57\,028&548 & -36&0(1) & -31&4(15) & .&. & .&. & -40&7(35) \\
150329\_C & 57\,111&334 & -52&0(1) & -53&1(19) & .&. & .&. & -54&4(45) \\
150830\_C & 57\,265&666 & -52&0(1) & -48&3(8) & -47&0(22) & -44&2(34) & -50&6(15) \\
150901\_C & 57\,267&659 & -44&4(1) & -43&2(8) & -35&1(21) & -39&0(38) & -39&8(16) \\
160721\_C & 57\,591&620 & -50&6(1) & -43&2(9) & -32&0(28) & -49&7(46) & -38&2(20) \\
170621\_S & 57\,926&683 & -63&4(1) & -59&5(11) & -17&8(53) & -64&8(48) & -58&9(28) \\
170718\_S & 57\,953&702 & -38&0(1) & -31&9(6) & -25&2(23) & -42&5(38) & -32&1(13) \\
190831\_I & 58\,727&677 & -64&4(1) & -61&9(3) & -62&2(5) & -56&0(16) & -61&1(6) \\
190901\_I & 58\,728&602 & -55&2(1) & -52&5(4) & -42&3(12) & -47&2(20) & -53&7(11) \\
190902\_I & 58\,729&663 & -47&2(1) & -44&4(5) & -35&5(9) & -42&7(21) & -41&4(11) \\
191012\_I & 58\,769&672 & -37&0(1) & -33&6(5) & -28&8(10) & -27&7(19) & -32&4(9) \\
191013\_I & 58\,770&594 & -35&4(1) & -31&1(6) & -25&5(11) & -29&0(22) & -30&2(12) \\
191014\_I & 58\,771&622 & -37&6(1) & -33&4(5) & -30&1(9) & -33&3(22) & -34&2(9) \\
191015\_I & 58\,772&528 & -49&0(1) & -45&7(5) & -44&9(11) & -41&1(22) & -37&6(13) \\
\hline  RV mean & .&. & -45&7 & -42&3 & -32&0 & -39&8 & -40&6 \\
$\sigma$ RV & .&. & 10&2 & 10&9 & 7&6 & 11&3 & 9&2 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for $\alpha$~Cam]{Radial velocity measurements for $\alpha$~Cam. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:alphaCam}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
041116\_P & 53\,326&584 & 6&0(1) & 8&8(13) & -15&8(7) & 12&3(15) & 13&5(5) & 15&0(6) \\
051107\_P & 53\,682&479 & 11&4(1) & 11&1(19) & -6&5(7) & 20&0(16) & 20&1(7) & 24&2(6) \\
081108\_I & 54\,779&573 & 7&8(1) & 10&3(13) & -9&3(6) & 15&1(11) & 18&4(4) & 16&8(5) \\
081108\_I\_2 & 54\,779&574 & 7&6(1) & 11&4(13) & -9&8(6) & 16&9(11) & 18&9(4) & 17&9(5) \\
081108\_I\_3 & 54\,779&576 & 7&8(1) & 9&1(14) & -9&3(6) & 16&8(11) & 17&5(5) & 18&8(5) \\
081108\_I\_4 & 54\,779&577 & 7&6(1) & 13&4(13) & -9&6(6) & 17&1(11) & 18&2(5) & 19&3(4) \\
081108\_I\_5 & 54\,779&578 & 7&8(1) & 11&3(13) & -9&5(6) & 15&1(10) & 16&6(4) & 17&7(5) \\
081108\_I\_6 & 54\,779&581 & 7&6(1) & 11&9(11) & -9&6(6) & 17&6(10) & 18&0(4) & 18&3(4) \\
110115\_I & 55\,577&490 & 13&4(1) & 12&4(12) & -6&3(5) & 15&7(11) & 20&5(5) & 19&9(5) \\
111108\_M & 55\,874&653 & 5&0(1) & 18&3(8) & -17&7(5) & 20&1(9) & 18&9(3) & 19&1(4) \\
120907\_C & 56\,178&680 & 5&2(1) & -2&6(24) & -10&5(8) & 11&3(15) & 15&1(7) & 16&4(5) \\
121223\_I & 56\,285&548 & 20&0(1) & 22&7(11) & -3&1(4) & 27&9(12) & 26&4(4) & 28&2(4) \\
121229\_C & 56\,291&590 & 10&0(1) & -0&0(32) & -10&7(6) & 23&4(18) & 24&1(9) & 24&8(7) \\
131025\_M & 56\,591&634 & 13&2(1) & 18&7(8) & -6&6(4) & 19&9(9) & 20&1(4) & 20&1(4) \\
131026\_M & 56\,592&509 & 16&6(1) & 14&3(8) & 0&5(5) & 16&5(9) & 17&2(3) & 20&6(4) \\
131027\_M & 56\,593&694 & 31&0(1) & 22&7(8) & 15&1(4) & 23&6(9) & 27&3(3) & 33&8(4) \\
131028\_M & 56\,594&672 & 18&6(1) & 14&6(9) & -0&6(5) & 20&4(10) & 22&2(4) & 22&1(5) \\
131029\_M & 56\,595&773 & 17&4(1) & 19&5(11) & -2&9(4) & 23&2(10) & 23&5(4) & 27&5(6) \\
131030\_M & 56\,596&715 & 8&2(1) & 12&1(13) & -7&0(5) & 12&9(11) & 13&0(5) & 13&7(6) \\
131213\_M & 56\,640&448 & 17&2(1) & 13&2(8) & 0&6(4) & 16&7(10) & 17&6(3) & 21&8(4) \\
131218\_M & 56\,645&331 & 14&4(1) & 18&8(7) & -3&7(4) & 20&0(9) & 20&5(3) & 25&6(3) \\
131219\_M & 56\,646&368 & 13&6(1) & 20&8(6) & -3&1(4) & 21&7(9) & 23&1(3) & 22&8(3) \\
131220\_M & 56\,647&343 & 13&2(1) & 24&8(9) & -8&4(4) & 24&2(9) & 24&2(4) & 30&0(4) \\
131220\_M\_2 & 56\,647&692 & 19&0(1) & 21&4(8) & 0&7(5) & 21&7(9) & 23&5(4) & 28&5(4) \\
131221\_M & 56\,648&376 & 17&0(1) & 16&7(8) & -1&0(4) & 17&8(9) & 20&8(4) & 23&3(4) \\
131221\_M\_2 & 56\,648&594 & 14&0(1) & 13&0(46) & -3&3(10) & 19&0(36) & 19&9(21) & 21&1(26) \\
131221\_M\_3 & 56\,648&717 & 12&0(1) & 10&5(26) & -5&5(7) & 14&8(29) & 16&9(13) & 22&0(15) \\
131222\_M & 56\,649&403 & 6&6(1) & 9&9(8) & -14&2(4) & 14&5(9) & 13&8(3) & 15&0(4) \\
131222\_M\_2 & 56\,649&607 & 0&8(1) & 11&6(7) & -19&5(5) & 14&9(9) & 13&3(3) & 14&1(4) \\
140311\_C & 56\,728&499 & 13&6(1) & 10&6(52) & -4&9(10) & 16&8(50) & 26&1(26) & 25&6(23) \\
141223\_P & 57\,015&323 & 15&8(1) & 11&3(10) & -4&2(3) & 26&4(9) & 24&6(4) & 22&9(4) \\
141223\_P\_2 & 57\,015&325 & 15&8(1) & 14&9(10) & -4&1(3) & 27&7(10) & 24&4(4) & 22&5(4) \\
161020\_C\_V & 57\,682&600 & 30&0(1) & 18&2(13) & 9&9(5) & .&. & 27&2(10) & 24&9(8) \\
161020\_C\_V\_2 & 57\,682&603 & 29&2(1) & 18&9(14) & 10&0(5) & .&. & 26&5(11) & 24&3(8) \\
161020\_C\_V\_3 & 57\,682&604 & 29&8(1) & 21&8(12) & 10&5(5) & .&. & 28&1(11) & 24&3(8) \\
161026\_C\_V & 57\,688&590 & 18&2(1) & 11&6(15) & -11&4(6) & .&. & 11&9(11) & 10&8(9) \\
171024\_M & 58\,051&768 & 9&2(1) & 16&6(6) & -9&7(4) & 16&7(8) & 17&9(3) & 20&0(5) \\
171111\_I & 58\,069&628 & 12&0(1) & 15&6(13) & -7&0(6) & 17&6(14) & 18&6(6) & 21&3(6) \\
171204\_M & 58\,092&748 & 9&4(1) & 15&2(5) & -8&5(4) & 14&7(8) & 15&3(2) & 19&0(3) \\
171205\_M & 58\,093&581 & 12&4(1) & 16&6(5) & -5&1(4) & 16&0(8) & 17&4(2) & 21&6(3) \\
171206\_M & 58\,094&530 & 17&0(1) & 20&4(4) & -3&2(4) & 19&9(8) & 21&9(2) & 26&2(3) \\
171207\_M & 58\,095&544 & 20&2(1) & 23&9(4) & 5&8(6) & 22&8(8) & 24&2(2) & 27&9(2) \\
171208\_M & 58\,096&577 & 16&8(1) & 22&0(5) & -2&7(4) & 21&6(8) & 22&6(2) & 26&2(3) \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\addtocounter{table}{-1}
\captionsetup[table]{list=no}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Continued.}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
171209\_M & 58\,097&483 & 30&2(1) & 29&0(5) & 12&8(3) & 27&0(8) & 28&8(2) & 34&9(3) \\
171210\_M & 58\,098&484 & 25&4(1) & 25&8(5) & 6&5(4) & 26&4(8) & 28&1(2) & 32&4(3) \\
171217\_M & 58\,105&438 & 18&8(1) & 17&2(5) & 1&1(4) & 17&6(8) & 20&2(2) & 23&4(3) \\
171218\_M & 58\,106&507 & 35&6(1) & 28&4(4) & 21&9(4) & 27&7(8) & 30&0(2) & 35&4(3) \\
171219\_M & 58\,107&518 & 21&4(1) & 22&4(5) & 2&9(5) & 22&0(8) & 24&6(2) & 29&9(3) \\
171221\_M & 58\,108&935 & 17&4(1) & 19&7(5) & -1&8(4) & 19&2(8) & 21&5(2) & 28&3(3) \\
181211\_S & 58\,464&359 & 6&4(1) & 14&7(14) & -18&1(10) & 19&6(13) & 18&7(6) & 19&9(6) \\
951109\_P & 50\,031&700 & 10&4(1) & 6&5(13) & -10&1(9) & 13&2(14) & 13&9(5) & 17&7(4) \\
\hline  RV mean & .&. & 15&0 & 16&1 & -4&4 & 19&2 & 20&7 & 22&7 \\
$\sigma$ RV & .&. & 7&7 & 5&8 & 7&7 & 4&3 & 4&6 & 5&4 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\captionsetup[table]{list=yes}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~37\,737]{Radial velocity measurements for HD~37\,737. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD37737}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
051109\_P & 53\,684&550 & -12&6(1) & -13&3(65) & -14&2(23) & .&. & .&. & -13&9(105) & .&. \\
130128\_I & 56\,321&476 & 10&2(1) & -8&3(7) & 10&1(5) & 20&8(9) & 31&6(22) & 33&8(14) & 36&1(13) \\
130129\_I & 56\,322&413 & 24&2(1) & 5&2(7) & 24&5(5) & 31&7(9) & 44&5(20) & 49&2(14) & 50&5(13) \\
130130\_I & 56\,323&497 & 30&6(1) & 11&2(8) & 31&1(6) & 38&3(9) & 47&6(21) & 53&5(14) & 50&1(16) \\
130215\_I & 56\,339&416 & 38&6(1) & 21&2(8) & 36&6(5) & 41&8(9) & 53&7(21) & 58&2(13) & 60&2(16) \\
171008\_I & 58\,035&713 & 9&2(1) & -9&8(8) & 7&4(6) & 11&5(8) & 22&9(21) & 26&1(12) & 35&6(16) \\
171030\_M & 58\,057&643 & 27&2(1) & 6&8(8) & 28&8(7) & 34&0(9) & 47&1(21) & 46&6(12) & 51&4(20) \\
171119\_I & 58\,077&730 & -61&0(1) & -78&8(10) & -61&4(7) & -53&3(14) & -65&1(36) & -38&6(22) & -34&3(25) \\
171120\_M & 58\,078&622 & -10&4(1) & -29&2(10) & -9&4(6) & -3&4(10) & -2&4(33) & 8&3(15) & 19&9(26) \\
171202\_I & 58\,090&503 & 16&2(1) & -4&9(15) & 17&5(9) & 14&6(17) & 31&1(43) & 36&4(30) & 41&0(42) \\
181212\_S & 58\,465&481 & 35&2(1) & 17&2(22) & 31&3(10) & 45&6(23) & 61&3(60) & 49&4(31) & 61&4(52) \\
190831\_I & 58\,727&714 & -74&6(1) & -95&8(15) & -73&6(8) & -77&4(13) & -92&2(46) & -81&7(24) & -130&6(38) \\
190902\_I & 58\,729&717 & -10&8(1) & -28&3(20) & -9&9(9) & -0&6(18) & -66&2(79) & 32&9(42) & -17&6(45) \\
191012\_I & 58\,769&690 & 9&2(1) & -6&9(16) & 6&8(11) & 10&4(22) & 20&9(53) & 31&0(33) & 18&1(57) \\
191013\_I & 58\,770&656 & 26&8(1) & 13&9(21) & 29&1(11) & 41&9(24) & 41&9(74) & 72&1(44) & 59&0(48) \\
191014\_I & 58\,771&656 & 30&8(1) & 11&3(18) & 34&2(11) & 35&4(21) & 27&9(66) & 61&7(39) & 38&8(52) \\
191015\_I & 58\,772&638 & 25&6(1) & 1&1(22) & 29&7(13) & 17&6(24) & 20&6(76) & 71&5(48) & 35&1(55) \\
\hline RV mean & .&. & 16&7 & -0&9 & 16&9 & 19&1 & 34&5 & 36&1 & 38&5 \\
$\sigma$ RV & .&. & 16&5 & 14&9 & 16&8 & 24&6 & 16&4 & 29&0 & 20&4 \\
Drop & .&. & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{3} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for 15~Mon~Aa]{Radial velocity measurements for 15~Mon~Aa. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:15MonAa}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4713}} & \multicolumn{2}{c}{\HeI{4922}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
951124\_P & 50\,046&528 & 27&8(1) & 32&5(3) & 25&0(6) & 30&5(8) & 32&0(3) & 32&4(5) & 31&7(3) & 31&7(4) \\
951128\_P & 50\,050&392 & 26&8(1) & 31&7(5) & 25&8(7) & 28&1(13) & 30&5(4) & 31&8(9) & 30&4(3) & 32&1(5) \\
951129\_P & 50\,051&600 & 28&0(1) & 33&6(6) & 26&3(5) & 28&7(7) & 32&0(3) & 33&2(6) & 32&2(4) & 30&9(9) \\
951130\_P & 50\,052&589 & 28&0(1) & 33&7(3) & 25&9(6) & 29&7(8) & 32&0(2) & 32&6(6) & 32&8(3) & 31&9(5) \\
951201\_P & 50\,053&653 & 27&4(1) & 33&0(3) & 26&9(7) & 29&6(8) & 31&6(3) & 32&1(7) & 31&6(3) & 31&8(3) \\
961118\_P & 50\,406&695 & 29&4(1) & 37&1(8) & 25&1(16) & 30&3(16) & 35&3(5) & 35&7(13) & 34&7(7) & 35&3(9) \\
961225\_P & 50\,443&463 & 30&4(1) & 35&4(3) & 28&1(6) & 32&9(7) & 34&8(3) & 36&3(6) & 35&2(4) & 35&6(3) \\
971109\_P & 50\,762&744 & 31&8(1) & 38&1(3) & 30&4(7) & 33&2(8) & 36&1(2) & 37&7(7) & 35&9(3) & 35&7(3) \\
971109\_P\_2 & 50\,762&753 & 31&6(1) & 37&2(3) & 29&0(7) & 32&8(8) & 35&7(2) & 37&6(7) & 35&8(3) & 35&8(3) \\
971112\_P & 50\,765&712 & 32&0(1) & 38&5(4) & 31&0(7) & 33&5(7) & 36&6(3) & 37&7(7) & 35&9(4) & 36&2(4) \\
041116\_P & 53\,326&640 & 30&6(1) & 35&4(3) & 28&9(7) & 34&0(7) & 34&6(2) & 34&6(8) & 34&0(3) & 34&8(3) \\
091109\_I & 55\,145&633 & 28&0(1) & 34&6(2) & 28&5(4) & 31&5(5) & 33&8(2) & 30&5(4) & 34&2(2) & 34&0(2) \\
100307\_F & 55\,263&642 & 28&8(1) & 33&7(6) & 26&9(5) & 32&0(5) & 33&2(3) & 34&1(4) & 31&7(3) & 34&3(3) \\
100307\_F\_2 & 55\,263&654 & 29&2(1) & 33&9(6) & 27&5(5) & 32&3(5) & 33&6(3) & 34&4(4) & 31&9(3) & 34&9(3) \\
110115\_I & 55\,577&628 & 29&2(1) & 34&2(3) & 28&1(5) & 32&0(5) & 33&9(2) & 32&7(5) & 33&9(2) & 35&0(3) \\
110909\_I & 55\,814&738 & 30&0(1) & 34&0(3) & 28&7(6) & 31&8(5) & 33&8(2) & 35&4(5) & 32&6(3) & 34&5(2) \\
121025\_M & 56\,226&694 & 29&4(1) & 35&2(3) & 27&0(5) & 31&5(6) & 33&9(2) & 34&0(4) & 33&1(2) & 35&2(3) \\
121025\_M\_2 & 56\,226&702 & 29&2(1) & 34&4(2) & 27&0(4) & 31&7(5) & 33&9(2) & 34&3(4) & 33&3(2) & 33&7(3) \\
121121\_C & 56\,253&695 & 27&2(1) & 34&1(4) & 28&2(6) & 29&4(7) & 33&5(2) & 35&6(6) & 34&0(4) & 34&2(4) \\
121223\_I & 56\,285&716 & 29&6(1) & 33&9(2) & 27&6(5) & 30&9(4) & 33&6(1) & 35&9(4) & 33&8(2) & 35&0(2) \\
121228\_C & 56\,290&479 & 28&2(1) & 35&5(4) & 28&9(7) & 31&5(8) & 34&4(2) & 36&0(7) & 34&1(4) & 35&4(3) \\
130129\_I & 56\,322&578 & 30&0(1) & 34&5(2) & 26&9(5) & 30&7(5) & 34&1(2) & 36&0(5) & 33&7(2) & 34&6(2) \\
130131\_C & 56\,324&511 & 26&6(1) & 34&2(7) & 27&6(6) & 30&1(7) & 33&6(2) & 39&0(10) & 35&5(4) & 34&2(4) \\
131207\_C & 56\,634&568 & 28&4(1) & 34&1(3) & 28&0(6) & 32&1(6) & 34&5(2) & 30&9(7) & 34&0(3) & 34&2(3) \\
151224\_I & 57\,381&568 & 29&0(1) & 35&5(3) & 25&9(7) & 33&5(7) & 31&1(2) & 36&0(5) & 34&5(3) & 35&5(3) \\
151224\_I\_2 & 57\,381&634 & 28&8(1) & 34&9(3) & 27&4(7) & 32&1(8) & 30&0(2) & 35&9(5) & 34&5(3) & 35&2(3) \\
151224\_I\_3 & 57\,381&678 & 31&2(1) & 35&1(3) & 26&9(8) & 35&5(7) & 34&5(2) & 36&5(6) & 35&7(2) & 36&0(3) \\
151224\_I\_4 & 57\,381&710 & 29&4(1) & 34&5(3) & 25&6(7) & 31&8(6) & 30&8(2) & 36&5(5) & 35&3(2) & 34&8(3) \\
151225\_I & 57\,382&459 & 29&4(1) & 34&6(3) & 26&6(7) & 31&6(7) & 33&0(2) & 34&7(5) & 33&0(3) & 34&1(3) \\
151225\_I\_2 & 57\,382&520 & 28&4(1) & 34&8(3) & 25&6(7) & 31&8(7) & 30&8(2) & 34&3(5) & 33&4(3) & 33&7(3) \\
151228\_I & 57\,385&415 & 28&0(1) & 33&1(3) & 24&2(7) & 31&1(7) & 30&6(2) & 33&4(5) & 32&7(3) & 33&5(3) \\
151228\_I\_10 & 57\,385&718 & 29&2(1) & 34&2(3) & 26&2(8) & 31&4(6) & 31&2(2) & 34&0(6) & 34&0(3) & 34&6(3) \\
151228\_I\_11 & 57\,385&725 & 29&4(1) & 35&0(3) & 25&4(7) & 33&0(7) & 31&2(2) & 34&9(6) & 33&9(3) & 34&2(2) \\
151228\_I\_12 & 57\,385&731 & 29&4(1) & 34&4(3) & 24&8(8) & 33&0(6) & 31&4(2) & 34&5(5) & 34&4(3) & 35&1(2) \\
151228\_I\_13 & 57\,385&737 & 29&6(1) & 34&8(3) & 27&2(8) & 33&0(7) & 31&5(2) & 35&0(6) & 34&1(2) & 34&7(3) \\
151228\_I\_14 & 57\,385&744 & 29&8(1) & 34&1(3) & 26&0(7) & 32&9(7) & 31&9(2) & 35&3(5) & 33&8(2) & 34&7(3) \\
151228\_I\_2 & 57\,385&476 & 29&0(1) & 34&4(3) & 23&7(8) & 32&2(7) & 31&3(2) & 35&1(5) & 33&6(2) & 34&1(3) \\
151228\_I\_3 & 57\,385&514 & 28&2(1) & 33&4(3) & 24&4(7) & 31&7(7) & 30&7(2) & 33&6(5) & 33&1(3) & 34&0(3) \\
151228\_I\_4 & 57\,385&546 & 28&2(1) & 33&6(3) & 25&1(8) & 31&5(7) & 31&0(2) & 33&7(5) & 33&4(2) & 33&5(3) \\
151228\_I\_5 & 57\,385&589 & 29&6(1) & 35&5(3) & 27&0(8) & 33&8(7) & 31&8(2) & 35&0(5) & 33&7(3) & 36&0(3) \\
151228\_I\_6 & 57\,385&626 & 28&6(1) & 33&9(3) & 27&2(8) & 32&7(7) & 30&7(2) & 35&4(5) & 33&7(3) & 34&7(2) \\
151228\_I\_7 & 57\,385&662 & 28&8(1) & 34&2(3) & 25&4(7) & 31&7(7) & 31&4(2) & 34&6(5) & 33&5(3) & 33&8(3) \\
151228\_I\_8 & 57\,385&682 & 30&2(1) & 33&8(3) & 25&4(7) & 32&5(7) & 34&4(2) & 34&5(5) & 33&3(3) & 34&2(3) \\
151228\_I\_9 & 57\,385&696 & 29&2(1) & 34&2(3) & 25&8(7) & 31&8(7) & 31&3(2) & 34&9(5) & 33&7(2) & 34&9(3) \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4143}, 4388, 4471, 4713, 5016, 5048, 5876, \HeII{4200}, 4542, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\captionsetup[table]{list=no}
\addtocounter{table}{-1}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Continued.}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeI{4713}} & \multicolumn{2}{c}{\HeI{4922}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
161026\_C\_V & 57\,688&658 & 32&6(1) & 34&2(4) & .&. & .&. & 33&1(2) & .&. & 32&6(5) & 31&6(5) \\
171217\_M & 58\,105&470 & 28&4(1) & 34&0(3) & 27&2(5) & 29&7(6) & 33&3(2) & 32&3(6) & 32&9(2) & 33&2(3) \\
171218\_M & 58\,106&694 & 29&0(1) & 35&0(3) & 26&6(4) & 32&3(4) & 33&8(1) & 32&9(4) & 33&2(2) & 33&9(3) \\
171219\_M & 58\,107&433 & 28&4(1) & 34&5(3) & 26&6(4) & 31&0(4) & 33&2(1) & 32&6(4) & 33&0(2) & 34&3(2) \\
171221\_M & 58\,109&055 & 28&2(1) & 34&1(2) & 26&9(3) & 31&0(4) & 33&1(1) & 32&4(3) & 32&6(1) & 33&6(1) \\
181124\_I & 58\,447&724 & 28&8(1) & 34&9(2) & 26&4(3) & 31&6(4) & 33&5(2) & 32&4(4) & 34&4(2) & 33&0(1) \\
181129\_I & 58\,452&737 & 28&6(1) & 33&8(5) & 26&7(9) & 30&5(7) & 34&6(3) & 30&9(6) & 35&0(4) & 32&7(5) \\
191013\_I & 58\,770&770 & 29&2(1) & 36&6(3) & 29&8(6) & 28&5(7) & 34&0(3) & 33&2(5) & 33&0(3) & 32&4(3) \\


\hline  RV mean & .&. & 29&1 & 34&3 & 26&8 & 31&6 & 32&9 & 34&4 & 33&7 & 34&2 \\
$\sigma$ RV & .&. & 1&1 & 0&7 & 1&5 & 1&3 & 1&6 & 1&8 & 1&1 & 1&1 \\
Drop & .&. & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{6} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}
\captionsetup[table]{list=yes}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~46\,573]{Radial velocity measurements for HD~46\,573. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD46573}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\NIII{4379}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
060104\_F & 53\,740&634 & 39&4(1) & 42&9(3) & 48&3(7) & 45&4(8) & 43&5(5) & 46&4(18) & 49&1(7) \\
060206\_F & 53\,773&580 & 37&0(1) & 40&4(2) & 45&3(4) & 43&0(8) & 41&2(4) & 45&4(7) & 47&7(5) \\
060206\_F\_2 & 53\,773&602 & 37&4(1) & 41&0(2) & 46&4(4) & 43&3(8) & 41&5(4) & 45&7(7) & 49&1(5) \\
110114\_I & 55\,576&483 & 57&8(1) & 61&7(2) & 65&7(4) & 60&4(9) & 62&9(5) & 66&9(14) & 65&9(6) \\
121223\_I & 56\,285&680 & 43&0(1) & 46&4(2) & 52&8(4) & 51&3(8) & 48&4(5) & 48&6(16) & 53&7(5) \\
121224\_I & 56\,286&625 & 41&6(1) & 43&3(2) & 49&9(4) & 49&0(9) & 48&5(5) & 48&1(18) & 53&1(7) \\
181124\_I & 58\,447&712 & 45&2(1) & 48&6(2) & 55&0(5) & 50&6(9) & 50&7(4) & 51&3(14) & 58&2(6) \\
181127\_I & 58\,450&653 & 37&0(1) & 41&1(2) & 47&6(5) & 42&5(9) & 44&1(5) & 46&4(16) & 47&5(7) \\
190318\_F & 58\,561&496 & 52&6(1) & 55&9(2) & 62&0(5) & 58&4(9) & 57&1(5) & 64&3(14) & 64&8(9) \\
190321\_F & 58\,564&485 & 42&8(1) & 46&2(2) & 51&2(5) & 49&7(8) & 47&5(5) & 49&3(12) & 54&0(8) \\
190322\_F & 58\,565&482 & 43&0(1) & 46&7(2) & 50&7(5) & 48&5(8) & 47&4(4) & 49&0(10) & 52&8(5) \\
190429\_S & 58\,603&382 & 56&0(1) & 58&2(3) & 61&4(8) & 64&5(12) & 61&6(7) & 64&6(17) & 61&2(12) \\
191012\_I & 58\,769&726 & 41&2(1) & 44&0(4) & 52&1(8) & 46&3(14) & 46&6(9) & 44&0(35) & 46&7(15) \\
191015\_I & 58\,772&741 & 55&4(1) & 60&4(4) & 64&2(8) & 61&1(14) & 64&2(9) & 68&3(31) & 64&7(14) \\
201012\_C\_V & 59\,135&658 & 55&4(1) & 57&7(2) & 63&7(3) & .&. & 60&6(7) & .&. & 59&9(11) \\
\hline  RV mean & .&. & 45&7 & 49&0 & 54&4 & 51&0 & 51&1 & 47&4 & 55&2 \\
$\sigma$ RV & .&. & 7&3 & 7&4 & 6&8 & 7&0 & 7&8 & 2&1 & 6&5 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0}0 & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{0} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{4471}, 5016, 5876, \HeII{4200}, 4542, 4686, 5412, H$\gamma$+\HeII{4338} and H$\beta$+\HeII{4860}.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for $\theta^{1}$~Ori~CaCb]{Radial velocity measurements for $\theta^{1}$~Ori~CaCb. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:theta^1OriCaCb}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
041119\_P & 53\,329&567 & 14&8(1) & 17&2(12) & 18&1(16) & 14&8(7) & 17&0(8) \\
060104\_F & 53\,741&034 & 26&2(1) & 27&3(3) & 25&7(6) & 23&4(4) & 27&2(3) \\
081107\_I & 54\,779&244 & 25&6(1) & 33&9(5) & 28&2(11) & 28&6(6) & 37&2(8) \\
081107\_I\_2 & 54\,779&253 & 26&0(1) & 34&1(2) & 31&3(5) & 27&2(4) & 32&9(3) \\
081108\_I & 54\,780&263 & 22&8(1) & 33&6(10) & 30&5(19) & 26&6(10) & 34&8(12) \\
110320\_F & 55\,642&070 & 31&0(1) & 41&3(10) & 39&4(10) & 30&5(8) & 43&7(9) \\
110320\_F\_2 & 55\,642&070 & 30&4(1) & 40&8(9) & 38&8(6) & 29&4(6) & 42&6(6) \\
110322\_F & 55\,644&030 & 27&6(1) & 40&4(9) & 38&4(6) & 30&1(6) & 42&8(5) \\
110909\_I & 55\,815&242 & 29&8(1) & 39&2(3) & 36&4(6) & 33&4(4) & 36&7(4) \\
121223\_I & 56\,286&096 & 34&8(1) & 47&0(2) & 45&2(5) & 41&8(4) & 46&1(3) \\
121229\_C & 56\,292&039 & 25&6(1) & 39&7(7) & 44&3(15) & 38&4(9) & 39&9(9) \\
130129\_I & 56\,322&973 & 31&4(1) & 46&2(2) & 47&0(6) & 39&8(4) & 45&1(3) \\
130131\_C & 56\,324&946 & 38&4(1) & 48&0(5) & 53&2(14) & 43&8(7) & 45&7(5) \\
131129\_C & 56\,627&147 & 24&0(1) & 26&1(4) & 18&2(15) & 20&7(7) & 24&3(6) \\
150330\_C & 57\,112&857 & 13&4(1) & 12&7(9) & 20&0(36) & 14&7(13) & 11&2(15) \\
151224\_I & 57\,382&064 & 20&8(1) & 19&5(3) & 20&8(7) & 19&0(4) & 20&5(4) \\
151228\_I & 57\,386&041 & 19&6(1) & 15&1(3) & 17&2(8) & 14&5(4) & 17&7(4) \\
160926\_M & 57\,659&209 & 19&6(1) & 19&0(3) & 16&7(6) & 16&6(3) & 17&4(4) \\
160928\_M & 57\,661&270 & 20&2(1) & 19&9(4) & 16&3(8) & 15&6(5) & 18&4(7) \\
160929\_M & 57\,662&270 & 20&6(1) & 19&9(4) & 17&4(8) & 14&8(4) & 20&0(6) \\
160930\_M & 57\,663&269 & 19&8(1) & 18&8(4) & 19&7(8) & 14&8(4) & 19&9(6) \\
161017\_M & 57\,680&213 & 21&6(1) & 22&0(2) & 21&9(6) & 18&0(3) & 22&7(3) \\
161018\_M & 57\,681&129 & 23&6(1) & 23&1(3) & 21&3(8) & 19&2(3) & 23&4(4) \\
161019\_M & 57\,682&151 & 26&2(1) & 22&8(2) & 22&8(6) & 20&2(3) & 21&7(3) \\
161020\_M & 57\,683&106 & 27&8(1) & 23&2(3) & 22&4(6) & 21&7(3) & 20&9(4) \\
161021\_M & 57\,684&059 & 26&0(1) & 24&5(8) & 20&7(8) & 22&9(5) & 20&8(5) \\
161022\_M & 57\,685&079 & 25&6(1) & 24&4(3) & 15&3(16) & 24&2(4) & 22&5(5) \\
171019\_M & 58\,047&110 & 25&4(1) & 29&7(3) & 25&4(5) & 23&3(3) & 27&1(4) \\
171020\_M & 58\,048&139 & 25&0(1) & 27&8(3) & 24&1(6) & 22&7(3) & 27&3(4) \\
171023\_M & 58\,051&227 & 25&4(1) & 27&3(3) & 24&0(6) & 23&1(3) & 27&1(4) \\
171024\_M & 58\,052&049 & 27&4(1) & 26&7(3) & 24&3(6) & 24&3(3) & 27&1(4) \\
171025\_M & 58\,053&249 & 28&6(1) & 27&8(2) & 24&3(5) & 25&5(3) & 25&2(3) \\
171026\_M & 58\,054&236 & 29&4(1) & 28&9(3) & 25&3(7) & 28&0(3) & 25&7(4) \\
171028\_M & 58\,056&129 & 28&4(1) & 28&6(2) & 26&8(5) & 28&7(2) & 27&1(2) \\
171029\_M & 58\,057&265 & 29&2(1) & 29&0(3) & 27&3(5) & 29&7(3) & 27&9(3) \\
171030\_M & 58\,058&209 & 28&6(1) & 29&9(2) & 26&6(5) & 29&5(3) & 28&7(3) \\
171120\_M & 58\,079&152 & 15&6(1) & 17&3(4) & 14&6(7) & 11&9(4) & 17&4(5) \\
171204\_M & 58\,093&063 & 23&6(1) & 26&2(3) & 22&1(5) & 21&2(3) & 24&6(4) \\
171205\_M & 58\,094&043 & 23&6(1) & 26&0(3) & 21&7(6) & 20&4(3) & 25&0(4) \\
171206\_M & 58\,095&199 & 22&6(1) & 25&4(3) & 22&1(5) & 19&4(3) & 24&8(4) \\
171207\_M & 58\,096&227 & 21&8(1) & 25&5(3) & 22&8(6) & 19&9(3) & 25&1(4) \\
171208\_M & 58\,097&224 & 24&0(1) & 24&8(8) & 23&8(20) & 23&8(8) & 22&3(12) \\
171209\_M & 58\,098&100 & 26&2(1) & 26&4(3) & 23&8(6) & 23&3(3) & 26&5(4) \\
171210\_M & 58\,099&111 & 27&8(1) & 27&2(3) & 24&8(6) & 24&1(3) & 25&1(4) \\
171217\_M & 58\,105&953 & 27&4(1) & 29&6(3) & 26&7(7) & 28&2(3) & 28&5(4) \\
171218\_M & 58\,107&179 & 27&6(1) & 30&2(2) & 27&4(6) & 25&5(3) & 29&3(4) \\
171219\_M & 58\,107&921 & 26&6(1) & 30&1(2) & 25&8(6) & 25&7(3) & 28&7(4) \\
171221\_M & 58\,109&612 & 25&4(1) & 28&5(3) & 24&8(5) & 23&0(3) & 27&7(4) \\
180920\_I & 58\,383&241 & 21&4(1) & 26&8(5) & 20&4(11) & 21&8(6) & 26&4(5) \\
180921\_I & 58\,384&148 & 18&2(1) & 25&6(8) & 17&5(28) & 17&5(11) & 24&8(12) \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeI{}+\HeII{4026}, \HeI{4388}, 4471, 4713, 4922, 5876, \HeII{4200}, 4542, and 5412.}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\captionsetup[table]{list=no}
\addtocounter{table}{-1}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption{Continued.}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\CIV{5812}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} & \multicolumn{2}{c}{\OIII{5592}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
181124\_I & 58\,448&181 & 19&0(1) & 22&6(2) & 16&7(7) & 18&7(4) & 20&1(3) \\
181125\_I & 58\,449&157 & 17&6(1) & 20&3(4) & 14&2(8) & 17&4(4) & 19&0(4) \\
181127\_I & 58\,451&100 & 14&8(1) & 19&1(3) & 15&0(8) & 13&8(4) & 17&7(5) \\
181128\_I & 58\,452&178 & 17&2(1) & 18&3(3) & 13&6(9) & 15&1(4) & 18&5(5) \\
181129\_I & 58\,453&126 & 19&6(1) & 19&7(4) & 14&3(9) & 17&4(5) & 17&9(5) \\
190831\_I & 58\,728&233 & 25&8(1) & 31&2(6) & .&. & .&. & .&. \\
190901\_I & 58\,729&254 & 30&4(1) & 30&5(27) & .&. & .&. & .&. \\
190902\_I & 58\,730&236 & 29&2(1) & 32&7(4) & .&. & .&. & .&. \\
191012\_I & 58\,770&246 & 27&6(1) & 34&2(5) & .&. & .&. & .&. \\
191013\_I & 58\,771&242 & 27&2(1) & 35&8(5) & .&. & .&. & .&. \\
191014\_I & 58\,772&239 & 27&8(1) & 33&2(5) & .&. & .&. & .&. \\
191015\_I & 58\,773&234 & 26&0(1) & 32&6(5) & .&. & .&. & .&. \\
951108\_P & 50\,030&599 & 18&6(1) & 19&3(3) & 18&5(7) & 15&1(5) & 18&9(4) \\
\hline  RV mean & .&. & 24&7 & 27&5 & 23&0 & 23&3 & 25&4 \\
$\sigma$ RV & .&. & 4&9 & 7&3 & 6&2 & 7&1 & 7&0 \\
Drop & .&. & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{3} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table*}

\captionsetup[table]{list=yes}
\begin{table*}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3} \tabcolsep=0.10cm
\caption[Radial velocity measurements for HD~52\,533~A]{Radial velocity measurements for HD~52\,533~A. Errors in parenthesis corresponds to the last digit.\\
\label{rvt:HD52533A}}
\begin{tabular}{l r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l  r@{.}l }
\hline \hline 
\multicolumn{1}{c}{Spectra} & \multicolumn{2}{c}{RJD} & \multicolumn{2}{c}{XCorr} & \multicolumn{2}{c}{\HeI{4471}} & \multicolumn{2}{c}{\HeI{5876}} & \multicolumn{2}{c}{\HeI{7065}} & \multicolumn{2}{c}{\HeII{4542}} & \multicolumn{2}{c}{\HeII{5412}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{d} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} & \multicolumn{2}{c}{km\,s$^{-1}$} \\
\hline
090501\_F & 54\,953&476 & -2&4(1) & 10&4(10) & -7&3(11) & 9&0(15) & -13&7(16) & -46&3(10) \\
110114\_I & 55\,576&630 & 140&2(1) & 116&2(25) & 147&5(20) & 151&7(31) & 232&9(28) & 204&2(14) \\
130215\_I & 56\,339&505 & 11&0(1) & 16&8(17) & 18&4(12) & 30&8(25) & 6&2(30) & 9&3(16) \\
140322\_C & 56\,739&411 & 103&4(1) & 51&8(85) & 114&3(52) & .&. & 137&0(104) & .&. \\
171001\_I & 58\,028&754 & 0&6(1) & -0&2(14) & 1&9(13) & 25&6(28) & -18&2(23) & -30&3(17) \\
171010\_S & 58\,037&693 & 127&2(1) & 59&3(42) & 146&1(26) & 206&6(59) & 168&9(47) & 157&7(33) \\
171106\_S & 58\,064&626 & 33&2(1) & -46&7(92) & 60&4(37) & 131&4(59) & .&. & .&. \\
171118\_S & 58\,076&593 & 27&4(1) & -40&7(70) & 49&8(37) & 111&4(65) & .&. & 6&5(57) \\
180418\_S & 58\,227&411 & -0&6(1) & -13&6(52) & 35&3(30) & 104&4(48) & .&. & -3&1(42) \\
181125\_I & 58\,448&669 & 18&6(1) & 1&5(12) & 28&9(11) & 27&3(18) & -4&3(22) & 25&2(12) \\
190102\_S & 58\,486&422 & -32&4(1) & 33&9(29) & 4&4(19) & 7&7(49) & 9&3(41) & -6&7(24) \\
190318\_F & 58\,561&508 & 67&4(1) & 48&9(12) & 65&7(15) & 84&3(24) & 107&4(22) & 92&2(14) \\
190322\_F & 58\,565&528 & 97&0(1) & 63&6(14) & 86&8(19) & 106&3(22) & 160&5(17) & 140&8(13) \\
191012\_I & 58\,769&766 & 16&0(1) & 15&7(27) & 15&4(19) & 7&9(43) & -11&6(45) & 13&7(30) \\
191015\_I & 58\,772&750 & 1&2(1) & -9&8(24) & 9&4(25) & -16&2(45) & -24&8(43) & 23&2(36) \\
\hline  RV mean & .&. & 26&2 & 20&5 & 51&8 & 70&6 & 20&8 & 8&4 \\
$\sigma$ RV & .&. & 38&6 & 41&4 & 49&5 & 64&2 & 55&6 & 35&2 \\
Drop & .&. & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{2} \\
\hline
\end{tabular}
\tablefoot{x-corr method lines: \HeII{4200}, 4542, 4686, 5412, 6560.}

\renewcommand{\arraystretch}{1.0}
\end{table*}


